Closure Relations for Shallow Granular Flows from Particle Simulations

The Discrete Particle Method (DPM) is used to model granular flows down an inclined chute. We observe three major regimes: static piles, steady uniform flows and accelerating flows. For flows over a smooth base, other (quasi-steady) regimes are observed where the flow is either highly energetic and strongly layered in depth for small inclinations, or non-uniform and oscillating for larger inclinations. For steady uniform flows, depth profiles of density, velocity and stress have been obtained using an improved coarse-graining method, which allows accurate statistics even at the base of the flow. A shallow-layer model for granular flows is completed with macro-scale closure relations obtained from micro-scale DPM simulations of steady flows. We thus obtain relations for the effective basal friction, shape factor, mean density, and the normal stress anisotropy as functions of layer thickness, flow velocity and basal roughness. For collisional flows, the functional dependencies are well determined and have been obtained.

==> CommentsStefan.tex <==
\begin{itemize}
\item Why not call it DEM? The name 'Elements' seems vague to me, DEM is already used for sth. else the the geophysics community.

\end{itemize}


==> Figures/A27NormalStressAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{zz}/p$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{xx}/p$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{yy}/p$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{zz}/p$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{15}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{25}%
\psfrag{x04}[t][t]{30}%
\psfrag{x05}[t][t]{35}%
\psfrag{x06}[t][t]{40}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.85}%
\psfrag{v02}[r][r]{0.9}%
\psfrag{v03}[r][r]{0.95}%
\psfrag{v04}[r][r]{1}%
\psfrag{v05}[r][r]{1.05}%
\psfrag{v06}[r][r]{1.1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{A27NormalStressAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End A27NormalStressAnisotropy.matlab.tex


==> Figures/A27V.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x/\bar{v}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=17.6$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=27.4$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=36.8$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.4}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.4}%
\psfrag{v09}[r][r]{1.6}%
\psfrag{v10}[r][r]{1.8}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{A27V.matlab.eps}}%
\end{psfrags}%
%
% End A27V.matlab.tex


==> Figures/A27dV.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x/v_B$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=36.8$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=17.6$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=27.4$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=36.8$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.8}%
\psfrag{v02}[r][r]{0.85}%
\psfrag{v03}[r][r]{0.9}%
\psfrag{v04}[r][r]{0.95}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{1.05}%
\psfrag{v07}[r][r]{1.1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{A27dV.matlab.eps}}%
\end{psfrags}%
%
% End A27dV.matlab.tex


==> Figures/Bpr.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$Ene_{kin}/Ene_{ela}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.25$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.5$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.65$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1.35$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1.5$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1.75$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s15}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s16}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{$10^{1}$}%
\psfrag{x02}[t][t]{$10^{2}$}%
\psfrag{x03}[t][t]{$10^{3}$}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{3}$}%
\psfrag{v02}[r][r]{$10^{4}$}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{Bpr.matlab.eps}}%
\end{psfrags}%
%
% End Bpr.matlab.tex


==> Figures/Bpr0.25_FlowruleFit.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_{stop}$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$u/\sqrt{gh}$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}fit: $1.0554x+0.020064$\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_{stop}(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$u/\sqrt{gh}$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$1.1085x+0.011576$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{50}%
\psfrag{x03}[t][t]{100}%
\psfrag{x04}[t][t]{150}%
\psfrag{x05}[t][t]{200}%
\psfrag{x06}[t][t]{250}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{50}%
\psfrag{x09}[t][t]{100}%
\psfrag{x10}[t][t]{150}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
\psfrag{v06}[r][r]{2.5}%
\psfrag{v07}[r][r]{3}%
\psfrag{v08}[r][r]{3.5}%
\psfrag{v09}[r][r]{4}%
\psfrag{v10}[r][r]{4.5}%
\psfrag{v11}[r][r]{0}%
\psfrag{v12}[r][r]{0.5}%
\psfrag{v13}[r][r]{1}%
\psfrag{v14}[r][r]{1.5}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{2.5}%
\psfrag{v17}[r][r]{3}%
\psfrag{v18}[r][r]{3.5}%
\psfrag{v19}[r][r]{4}%
\psfrag{v20}[r][r]{4.5}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{Bpr0.25_FlowruleFit.matlab.eps}}%
\end{psfrags}%
%
% End Bpr0.25_FlowruleFit.matlab.tex


==> Figures/Bpr0.25_HStopFit.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h_{stop}, \theta_1=18.9706, \theta_2=25, Ad=0.51835$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{19}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{21}%
\psfrag{x04}[t][t]{22}%
\psfrag{x05}[t][t]{23}%
\psfrag{x06}[t][t]{24}%
\psfrag{x07}[t][t]{25}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
\psfrag{v09}[r][r]{40}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{Bpr0.25_HStopFit.matlab.eps}}%
\end{psfrags}%
%
% End Bpr0.25_HStopFit.matlab.tex


==> Figures/Bpr0.375_FlowruleFit.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_{stop}$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$u/\sqrt{gh}$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}fit: $-0.064437x+0.092954$\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_{stop}(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$u/\sqrt{gh}$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-0.040147x+0.055999$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{4}%
\psfrag{x08}[t][t]{6}%
\psfrag{x09}[t][t]{8}%
\psfrag{x10}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{0}%
\psfrag{v12}[r][r]{0.1}%
\psfrag{v13}[r][r]{0.2}%
\psfrag{v14}[r][r]{0.3}%
\psfrag{v15}[r][r]{0.4}%
\psfrag{v16}[r][r]{0.5}%
\psfrag{v17}[r][r]{0.6}%
\psfrag{v18}[r][r]{0.7}%
\psfrag{v19}[r][r]{0.8}%
\psfrag{v20}[r][r]{0.9}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{Bpr0.375_FlowruleFit.matlab.eps}}%
\end{psfrags}%
%
% End Bpr0.375_FlowruleFit.matlab.tex


==> Figures/Bpr0.375_HStopFit.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h_{stop}, \theta_1=19.3454, \theta_2=26.5089, Ad=3.1125$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{19}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{21}%
\psfrag{x04}[t][t]{22}%
\psfrag{x05}[t][t]{23}%
\psfrag{x06}[t][t]{24}%
\psfrag{x07}[t][t]{25}%
\psfrag{x08}[t][t]{26}%
\psfrag{x09}[t][t]{27}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{Bpr0.375_HStopFit.matlab.eps}}%
\end{psfrags}%
%
% End Bpr0.375_HStopFit.matlab.tex


==> Figures/Bpr0.5_FlowruleFit.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_{stop}$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$u/\sqrt{gh}$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}fit: $-0.13262x+0.14518$\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_{stop}(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$u/\sqrt{gh}$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-0.058972x+0.068434$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{30}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{5}%
\psfrag{x07}[t][t]{10}%
\psfrag{x08}[t][t]{15}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.4}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.4}%
\psfrag{v09}[r][r]{1.6}%
\psfrag{v10}[r][r]{1.8}%
\psfrag{v11}[r][r]{2}%
\psfrag{v12}[r][r]{0}%
\psfrag{v13}[r][r]{0.2}%
\psfrag{v14}[r][r]{0.4}%
\psfrag{v15}[r][r]{0.6}%
\psfrag{v16}[r][r]{0.8}%
\psfrag{v17}[r][r]{1}%
\psfrag{v18}[r][r]{1.2}%
\psfrag{v19}[r][r]{1.4}%
\psfrag{v20}[r][r]{1.6}%
\psfrag{v21}[r][r]{1.8}%
\psfrag{v22}[r][r]{2}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{Bpr0.5_FlowruleFit.matlab.eps}}%
\end{psfrags}%
%
% End Bpr0.5_FlowruleFit.matlab.tex


==> Figures/Bpr0.5_HStopFit.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h_{stop}, \theta_1=19.3483, \theta_2=38.6507, Ad=0.99601$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{15}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{25}%
\psfrag{x04}[t][t]{30}%
\psfrag{x05}[t][t]{35}%
\psfrag{x06}[t][t]{40}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{Bpr0.5_HStopFit.matlab.eps}}%
\end{psfrags}%
%
% End Bpr0.5_HStopFit.matlab.tex


==> Figures/Bpr21Ene.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$E_{kin}/E_{ela}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{$10^{1}$}%
\psfrag{x02}[t][t]{$10^{2}$}%
\psfrag{x03}[t][t]{$10^{3}$}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{2}$}%
\psfrag{v02}[r][r]{$10^{3}$}%
\psfrag{v03}[r][r]{$10^{4}$}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{Bpr21Ene.matlab.eps}}%
\end{psfrags}%
%
% End Bpr21Ene.matlab.tex


==> Figures/Bpr21Nu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.75$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.25$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.5$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.75$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{0.52}%
\psfrag{v03}[r][r]{0.54}%
\psfrag{v04}[r][r]{0.56}%
\psfrag{v05}[r][r]{0.58}%
\psfrag{v06}[r][r]{0.6}%
\psfrag{v07}[r][r]{0.62}%
\psfrag{v08}[r][r]{0.64}%
\psfrag{v09}[r][r]{0.66}%
\psfrag{v10}[r][r]{0.68}%
\psfrag{v11}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{Bpr21Nu.matlab.eps}}%
\end{psfrags}%
%
% End Bpr21Nu.matlab.tex


==> Figures/Bpr21VelocityX.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x/\bar{v}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.2}%
\psfrag{v02}[r][r]{0.4}%
\psfrag{v03}[r][r]{0.6}%
\psfrag{v04}[r][r]{0.8}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{1.2}%
\psfrag{v07}[r][r]{1.4}%
\psfrag{v08}[r][r]{1.6}%
\psfrag{v09}[r][r]{1.8}%
\psfrag{v10}[r][r]{2}%
\psfrag{v11}[r][r]{2.2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{Bpr21VelocityX.matlab.eps}}%
\end{psfrags}%
%
% End Bpr21VelocityX.matlab.tex


==> Figures/Bpr21W0.5Nu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{Bpr21W0.5Nu.matlab.eps}}%
\end{psfrags}%
%
% End Bpr21W0.5Nu.matlab.tex


==> Figures/BprEne.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$E_{kin}/E_{ela}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{$10^{1}$}%
\psfrag{x02}[t][t]{$10^{2}$}%
\psfrag{x03}[t][t]{$10^{3}$}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{3}$}%
\psfrag{v02}[r][r]{$10^{4}$}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{BprEne.matlab.eps}}%
\end{psfrags}%
%
% End BprEne.matlab.tex


==> Figures/BprHstop.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=.25$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=.5$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=.375$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=.25$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{18}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{24}%
\psfrag{x05}[t][t]{26}%
\psfrag{x06}[t][t]{28}%
\psfrag{x07}[t][t]{30}%
\psfrag{x08}[t][t]{32}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
\psfrag{v09}[r][r]{40}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{BprHstop.matlab.eps}}%
\end{psfrags}%
%
% End BprHstop.matlab.tex


==> Figures/BprLegend.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.25$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.5$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.65$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1.35$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1.5$}%
\psfrag{s15}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1.75$}%
\psfrag{s16}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s17}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s18}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
\psfrag{x12}[t][t]{2}%
\psfrag{x13}[t][t]{4}%
\psfrag{x14}[t][t]{6}%
\psfrag{x15}[t][t]{8}%
\psfrag{x16}[t][t]{10}%
\psfrag{x17}[t][t]{12}%
\psfrag{x18}[t][t]{14}%
\psfrag{x19}[t][t]{16}%
\psfrag{x20}[t][t]{18}%
\psfrag{x21}[t][t]{20}%
\psfrag{x22}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{1}%
\psfrag{v12}[r][r]{0}%
\psfrag{v13}[r][r]{0.1}%
\psfrag{v14}[r][r]{0.2}%
\psfrag{v15}[r][r]{0.3}%
\psfrag{v16}[r][r]{0.4}%
\psfrag{v17}[r][r]{0.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{BprLegend.matlab.eps}}%
\end{psfrags}%
%
% End BprLegend.matlab.tex


==> Figures/BprNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{0.51}%
\psfrag{v03}[r][r]{0.52}%
\psfrag{v04}[r][r]{0.53}%
\psfrag{v05}[r][r]{0.54}%
\psfrag{v06}[r][r]{0.55}%
\psfrag{v07}[r][r]{0.56}%
\psfrag{v08}[r][r]{0.57}%
\psfrag{v09}[r][r]{0.58}%
\psfrag{v10}[r][r]{0.59}%
\psfrag{v11}[r][r]{0.6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{BprNu.matlab.eps}}%
\end{psfrags}%
%
% End BprNu.matlab.tex


==> Figures/BprVelocityX.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x/\bar{v}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.4}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.4}%
\psfrag{v09}[r][r]{1.6}%
\psfrag{v10}[r][r]{1.8}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{BprVelocityX.matlab.eps}}%
\end{psfrags}%
%
% End BprVelocityX.matlab.tex


==> Figures/BprW0.5Nu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.45}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{0.55}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.65}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{BprW0.5Nu.matlab.eps}}%
\end{psfrags}%
%
% End BprW0.5Nu.matlab.tex


==> Figures/CubicDensity.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{1.5}%
\psfrag{x05}[t][t]{2}%
\psfrag{x06}[t][t]{2.5}%
\psfrag{x07}[t][t]{3}%
\psfrag{x08}[t][t]{3.5}%
\psfrag{x09}[t][t]{4}%
\psfrag{x10}[t][t]{4.5}%
\psfrag{x11}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{0.6}%
\psfrag{v03}[r][r]{0.7}%
\psfrag{v04}[r][r]{0.8}%
\psfrag{v05}[r][r]{0.9}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.1}%
\psfrag{v08}[r][r]{1.2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{CubicDensity.matlab.eps}}%
\end{psfrags}%
%
% End CubicDensity.matlab.tex


==> Figures/CubicNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}macro-prediction}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}simulation}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}macro-prediction}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{1.5}%
\psfrag{x05}[t][t]{2}%
\psfrag{x06}[t][t]{2.5}%
\psfrag{x07}[t][t]{3}%
\psfrag{x08}[t][t]{3.5}%
\psfrag{x09}[t][t]{4}%
\psfrag{x10}[t][t]{4.5}%
\psfrag{x11}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.25}%
\psfrag{v02}[r][r]{0.3}%
\psfrag{v03}[r][r]{0.35}%
\psfrag{v04}[r][r]{0.4}%
\psfrag{v05}[r][r]{0.45}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.55}%
\psfrag{v08}[r][r]{0.6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{CubicNu.matlab.eps}}%
\end{psfrags}%
%
% End CubicNu.matlab.tex


==> Figures/CubicStressZZ.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{zz}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}macro-prediction}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}simulation}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}macro-prediction}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{1.5}%
\psfrag{x05}[t][t]{2}%
\psfrag{x06}[t][t]{2.5}%
\psfrag{x07}[t][t]{3}%
\psfrag{x08}[t][t]{3.5}%
\psfrag{x09}[t][t]{4}%
\psfrag{x10}[t][t]{4.5}%
\psfrag{x11}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
\psfrag{v06}[r][r]{2.5}%
\psfrag{v07}[r][r]{3}%
\psfrag{v08}[r][r]{3.5}%
\psfrag{v09}[r][r]{4}%
\psfrag{v10}[r][r]{4.5}%
\psfrag{v11}[r][r]{5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{CubicStressZZ.matlab.eps}}%
\end{psfrags}%
%
% End CubicStressZZ.matlab.tex


==> Figures/EneRatio.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$Ene_{kin}/Ene_{ela}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=16.4, \theta=20^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=257, \theta=31^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=21.4, \theta=30^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=17.8, \theta=27^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=17.3, \theta=25^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=16.9, \theta=23^\circ$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=16.7, \theta=22^\circ$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=16.6, \theta=21^\circ$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=16.4, \theta=20^\circ$}%
\psfrag{s15}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s16}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{$10^{1}$}%
\psfrag{x02}[t][t]{$10^{2}$}%
\psfrag{x03}[t][t]{$10^{3}$}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{0}$}%
\psfrag{v02}[r][r]{$10^{2}$}%
\psfrag{v03}[r][r]{$10^{4}$}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{EneRatio.matlab.eps}}%
\end{psfrags}%
%
% End EneRatio.matlab.tex


==> Figures/Flowrule.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}h/h_{stop}*tan(\theta)^2\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}F\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}PJ-Flow rule (\theta=20-30^\circ)\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}h\approx h_{acc}}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}h=10}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}h=20}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}h=30}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}h\approx h_{acc}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{1.5}%
\psfrag{x05}[t][t]{2}%
\psfrag{x06}[t][t]{2.5}%
\psfrag{x07}[t][t]{3}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{Flowrule.matlab.eps}}%
\end{psfrags}%
%
% End Flowrule.matlab.tex


==> Figures/FlowruleFit.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_{stop}$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$u/\sqrt{gh}$\end{tabular}}%
\psfrag{s03}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_{stop}(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$u/\sqrt{gh}$\end{tabular}}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h\approx h_{acc}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=7.5$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=17.5$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=27.5$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h\approx h_{stop}$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h\approx h_{acc}$}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s15}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{30}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{5}%
\psfrag{x07}[t][t]{10}%
\psfrag{x08}[t][t]{15}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
\psfrag{v06}[r][r]{0}%
\psfrag{v07}[r][r]{0.5}%
\psfrag{v08}[r][r]{1}%
\psfrag{v09}[r][r]{1.5}%
\psfrag{v10}[r][r]{2}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{FlowruleFit.matlab.eps}}%
\end{psfrags}%
%
% End FlowruleFit.matlab.tex


==> Figures/H20Energy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$E_{kin}/E_{ela}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{10}%
\psfrag{x02}[t][t]{100}%
\psfrag{x03}[t][t]{200}%
\psfrag{x04}[t][t]{300}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{-6}$}%
\psfrag{v02}[r][r]{$10^{-4}$}%
\psfrag{v03}[r][r]{$10^{-2}$}%
\psfrag{v04}[r][r]{$10^{0}$}%
\psfrag{v05}[r][r]{$10^{2}$}%
\psfrag{v06}[r][r]{$10^{4}$}%
%
% Figure:
\resizebox{7cm}{!}{\includegraphics{H20Energy.matlab.eps}}%
\end{psfrags}%
%
% End H20Energy.matlab.tex


==> Figures/H20EnergyInlay.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$E_{kin}/E_{ela}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{$10^{2}$}%
\psfrag{x02}[t][t]{$10^{3}$}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{3}$}%
\psfrag{v02}[r][r]{$10^{4}$}%
%
% Figure:
\resizebox{7cm}{!}{\includegraphics{H20EnergyInlay.matlab.eps}}%
\end{psfrags}%
%
% End H20EnergyInlay.matlab.tex


==> Figures/H20EnergyLegend.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$Ene_{kin}/Ene_{ela}$\end{tabular}}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$31^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$20^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$20.5^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$21^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$21.5^\circ$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$23^\circ$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$24^\circ$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$25^\circ$}%
\psfrag{s15}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$27^\circ$}%
\psfrag{s16}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$28^\circ$}%
\psfrag{s17}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$29^\circ$}%
\psfrag{s18}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$30^\circ$}%
\psfrag{s19}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$31^\circ$}%
\psfrag{s20}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s21}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
\psfrag{x12}[t][t]{$10^{1}$}%
\psfrag{x13}[t][t]{$10^{2}$}%
\psfrag{x14}[t][t]{$10^{3}$}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{1}%
\psfrag{v12}[r][r]{$10^{-6}$}%
\psfrag{v13}[r][r]{$10^{-4}$}%
\psfrag{v14}[r][r]{$10^{-2}$}%
\psfrag{v15}[r][r]{$10^{0}$}%
\psfrag{v16}[r][r]{$10^{2}$}%
\psfrag{v17}[r][r]{$10^{4}$}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{H20EnergyLegend.matlab.eps}}%
\end{psfrags}%
%
% End H20EnergyLegend.matlab.tex


==> Figures/H20NormalStressAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$(\sigma_{zz}/p)_{flow}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$(\sigma_{xx}/p)_{flow}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$(\sigma_{yy}/p)_{flow}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$(\sigma_{zz}/p)_{flow}$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{23}%
\psfrag{x02}[t][t]{23.5}%
\psfrag{x03}[t][t]{24}%
\psfrag{x04}[t][t]{24.5}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{25.5}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{26.5}%
\psfrag{x09}[t][t]{27}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.85}%
\psfrag{v02}[r][r]{0.9}%
\psfrag{v03}[r][r]{0.95}%
\psfrag{v04}[r][r]{1}%
\psfrag{v05}[r][r]{1.05}%
\psfrag{v06}[r][r]{1.1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{H20NormalStressAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End H20NormalStressAnisotropy.matlab.tex


==> Figures/H20Nu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.4}%
\psfrag{v02}[r][r]{0.42}%
\psfrag{v03}[r][r]{0.44}%
\psfrag{v04}[r][r]{0.46}%
\psfrag{v05}[r][r]{0.48}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.52}%
\psfrag{v08}[r][r]{0.54}%
\psfrag{v09}[r][r]{0.56}%
\psfrag{v10}[r][r]{0.58}%
\psfrag{v11}[r][r]{0.6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{H20Nu.matlab.eps}}%
\end{psfrags}%
%
% End H20Nu.matlab.tex


==> Figures/H20P.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{zz}/mg$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{H20P.matlab.eps}}%
\end{psfrags}%
%
% End H20P.matlab.tex


==> Figures/H20V.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{H20V.matlab.eps}}%
\end{psfrags}%
%
% End H20V.matlab.tex


==> Figures/H40V.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x/\bar{v}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.4}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.4}%
\psfrag{v09}[r][r]{1.6}%
\psfrag{v10}[r][r]{1.8}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{H40V.matlab.eps}}%
\end{psfrags}%
%
% End H40V.matlab.tex


==> Figures/H40dV.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x/v_B$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.8}%
\psfrag{v02}[r][r]{0.85}%
\psfrag{v03}[r][r]{0.9}%
\psfrag{v04}[r][r]{0.95}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{1.05}%
\psfrag{v07}[r][r]{1.1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{H40dV.matlab.eps}}%
\end{psfrags}%
%
% End H40dV.matlab.tex


==> Figures/HPrincipalStressAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=27}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=9}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=18}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=27}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{23}%
\psfrag{x02}[t][t]{23.5}%
\psfrag{x03}[t][t]{24}%
\psfrag{x04}[t][t]{24.5}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{25.5}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{26.5}%
\psfrag{x09}[t][t]{27}%
%
% yticklabels:
\psfrag{v01}[r][r]{44.6}%
\psfrag{v02}[r][r]{44.8}%
\psfrag{v03}[r][r]{45}%
\psfrag{v04}[r][r]{45.2}%
\psfrag{v05}[r][r]{45.4}%
\psfrag{v06}[r][r]{45.6}%
\psfrag{v07}[r][r]{45.8}%
\psfrag{v08}[r][r]{46}%
\psfrag{v09}[r][r]{46.2}%
\psfrag{v10}[r][r]{46.4}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{HPrincipalStressAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End HPrincipalStressAnisotropy.matlab.tex


==> Figures/HStopFit.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h_{stop}, \theta_1=19.3953, \theta_2=39.057, h=0.95058$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{18}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{24}%
\psfrag{x05}[t][t]{26}%
\psfrag{x06}[t][t]{28}%
\psfrag{x07}[t][t]{30}%
\psfrag{x08}[t][t]{32}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
%
% Figure:
\resizebox{12cm}{!}{\includegraphics{HStopFit.matlab.eps}}%
\end{psfrags}%
%
% End HStopFit.matlab.tex


==> Figures/Mu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}s01\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}s02\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}s06\end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}s07\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{x01}%
\psfrag{x02}[t][t]{x02}%
\psfrag{x03}[t][t]{x03}%
\psfrag{x04}[t][t]{x04}%
\psfrag{x05}[t][t]{x05}%
\psfrag{x06}[t][t]{x06}%
\psfrag{x07}[t][t]{x07}%
\psfrag{x08}[t][t]{x08}%
\psfrag{x09}[t][t]{x09}%
\psfrag{x10}[t][t]{x10}%
%
% yticklabels:
\psfrag{v01}[r][r]{v01}%
\psfrag{v02}[r][r]{v02}%
\psfrag{v03}[r][r]{v03}%
\psfrag{v04}[r][r]{v04}%
\psfrag{v05}[r][r]{v05}%
\psfrag{v06}[r][r]{v06}%
\psfrag{v07}[r][r]{v07}%
\psfrag{v08}[r][r]{v08}%
\psfrag{v09}[r][r]{v09}%
\psfrag{v10}[r][r]{v10}%
\psfrag{v11}[r][r]{v11}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{Mu.matlab.eps}}%
\end{psfrags}%
%
% End Mu.matlab.tex


==> Figures/MuEnergy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$E_{kin}/E_{ela}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{$10^{1}$}%
\psfrag{x02}[t][t]{$10^{2}$}%
\psfrag{x03}[t][t]{$10^{3}$}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{3}$}%
\psfrag{v02}[r][r]{$10^{4}$}%
\psfrag{v03}[r][r]{$10^{5}$}%
\psfrag{v04}[r][r]{$10^{6}$}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{MuEnergy.matlab.eps}}%
\end{psfrags}%
%
% End MuEnergy.matlab.tex


==> Figures/MuLegend.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=8$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=0.25$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=0.5$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=1$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=2$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=4$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=8$}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s15}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{5}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{15}%
\psfrag{x04}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
%
% Figure:
\resizebox{7cm}{!}{\includegraphics{MuLegend.matlab.eps}}%
\end{psfrags}%
%
% End MuLegend.matlab.tex


==> Figures/MuMu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}/\sigma_{zz}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.4}%
\psfrag{v02}[r][r]{0.41}%
\psfrag{v03}[r][r]{0.42}%
\psfrag{v04}[r][r]{0.43}%
\psfrag{v05}[r][r]{0.44}%
\psfrag{v06}[r][r]{0.45}%
\psfrag{v07}[r][r]{0.46}%
\psfrag{v08}[r][r]{0.47}%
\psfrag{v09}[r][r]{0.48}%
\psfrag{v10}[r][r]{0.49}%
\psfrag{v11}[r][r]{0.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{MuMu.matlab.eps}}%
\end{psfrags}%
%
% End MuMu.matlab.tex


==> Figures/MuNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{0.51}%
\psfrag{v03}[r][r]{0.52}%
\psfrag{v04}[r][r]{0.53}%
\psfrag{v05}[r][r]{0.54}%
\psfrag{v06}[r][r]{0.55}%
\psfrag{v07}[r][r]{0.56}%
\psfrag{v08}[r][r]{0.57}%
\psfrag{v09}[r][r]{0.58}%
\psfrag{v10}[r][r]{0.59}%
\psfrag{v11}[r][r]{0.6}%
%
% Figure:
\resizebox{7cm}{!}{\includegraphics{MuNu.matlab.eps}}%
\end{psfrags}%
%
% End MuNu.matlab.tex


==> Figures/MuSd.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$Sd$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.4}%
\psfrag{v02}[r][r]{0.41}%
\psfrag{v03}[r][r]{0.42}%
\psfrag{v04}[r][r]{0.43}%
\psfrag{v05}[r][r]{0.44}%
\psfrag{v06}[r][r]{0.45}%
\psfrag{v07}[r][r]{0.46}%
\psfrag{v08}[r][r]{0.47}%
\psfrag{v09}[r][r]{0.48}%
\psfrag{v10}[r][r]{0.49}%
\psfrag{v11}[r][r]{0.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{MuSd.matlab.eps}}%
\end{psfrags}%
%
% End MuSd.matlab.tex


==> Figures/MuSdStar.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$Sd^\star$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.4}%
\psfrag{v02}[r][r]{0.41}%
\psfrag{v03}[r][r]{0.42}%
\psfrag{v04}[r][r]{0.43}%
\psfrag{v05}[r][r]{0.44}%
\psfrag{v06}[r][r]{0.45}%
\psfrag{v07}[r][r]{0.46}%
\psfrag{v08}[r][r]{0.47}%
\psfrag{v09}[r][r]{0.48}%
\psfrag{v10}[r][r]{0.49}%
\psfrag{v11}[r][r]{0.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{MuSdStar.matlab.eps}}%
\end{psfrags}%
%
% End MuSdStar.matlab.tex


==> Figures/MuVelocityX.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{1}%
\psfrag{v02}[r][r]{2}%
\psfrag{v03}[r][r]{3}%
\psfrag{v04}[r][r]{4}%
\psfrag{v05}[r][r]{5}%
\psfrag{v06}[r][r]{6}%
\psfrag{v07}[r][r]{7}%
%
% Figure:
\resizebox{7cm}{!}{\includegraphics{MuVelocityX.matlab.eps}}%
\end{psfrags}%
%
% End MuVelocityX.matlab.tex


==> Figures/NormalEnergy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$E_{kin}/E_{ela}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=15^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=0^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=6^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=15^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{$10^{1}$}%
\psfrag{x02}[t][t]{$10^{2}$}%
\psfrag{x03}[t][t]{$10^{3}$}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{-8}$}%
\psfrag{v02}[r][r]{$10^{-6}$}%
\psfrag{v03}[r][r]{$10^{-4}$}%
\psfrag{v04}[r][r]{$10^{-2}$}%
\psfrag{v05}[r][r]{$10^{0}$}%
\psfrag{v06}[r][r]{$10^{2}$}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalEnergy.matlab.eps}}%
\end{psfrags}%
%
% End NormalEnergy.matlab.tex


==> Figures/NormalFlowVelocity.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=15^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=0^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=6^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=15^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalFlowVelocity.matlab.eps}}%
\end{psfrags}%
%
% End NormalFlowVelocity.matlab.tex


==> Figures/NormalMu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$atan(-\sigma_{xz}/\sigma_{zz})$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=15^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=0^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=6^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=15^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{2}%
\psfrag{v03}[r][r]{4}%
\psfrag{v04}[r][r]{6}%
\psfrag{v05}[r][r]{8}%
\psfrag{v06}[r][r]{10}%
\psfrag{v07}[r][r]{12}%
\psfrag{v08}[r][r]{14}%
\psfrag{v09}[r][r]{16}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalMu.matlab.eps}}%
\end{psfrags}%
%
% End NormalMu.matlab.tex


==> Figures/NormalNormalPressureAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{ii}/p$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=0^\circ$\end{tabular}}%
\psfrag{s05}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{ii}/p$\end{tabular}}%
\psfrag{s08}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=6^\circ$\end{tabular}}%
\psfrag{s09}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s11}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{ii}/p$\end{tabular}}%
\psfrag{s13}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=15^\circ$\end{tabular}}%
\psfrag{s16}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s17}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s18}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s19}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s20}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s21}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{0.5}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{0.5}%
\psfrag{x09}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.9}%
\psfrag{v02}[r][r]{0.92}%
\psfrag{v03}[r][r]{0.94}%
\psfrag{v04}[r][r]{0.96}%
\psfrag{v05}[r][r]{0.98}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.02}%
\psfrag{v08}[r][r]{1.04}%
\psfrag{v09}[r][r]{1.06}%
\psfrag{v10}[r][r]{1.08}%
\psfrag{v11}[r][r]{1.1}%
\psfrag{v12}[r][r]{0.9}%
\psfrag{v13}[r][r]{0.92}%
\psfrag{v14}[r][r]{0.94}%
\psfrag{v15}[r][r]{0.96}%
\psfrag{v16}[r][r]{0.98}%
\psfrag{v17}[r][r]{1}%
\psfrag{v18}[r][r]{1.02}%
\psfrag{v19}[r][r]{1.04}%
\psfrag{v20}[r][r]{1.06}%
\psfrag{v21}[r][r]{1.08}%
\psfrag{v22}[r][r]{1.1}%
\psfrag{v23}[r][r]{0.9}%
\psfrag{v24}[r][r]{0.92}%
\psfrag{v25}[r][r]{0.94}%
\psfrag{v26}[r][r]{0.96}%
\psfrag{v27}[r][r]{0.98}%
\psfrag{v28}[r][r]{1}%
\psfrag{v29}[r][r]{1.02}%
\psfrag{v30}[r][r]{1.04}%
\psfrag{v31}[r][r]{1.06}%
\psfrag{v32}[r][r]{1.08}%
\psfrag{v33}[r][r]{1.1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalNormalPressureAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End NormalNormalPressureAnisotropy.matlab.tex


==> Figures/NormalNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=15^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=0^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=6^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=15^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalNu.matlab.eps}}%
\end{psfrags}%
%
% End NormalNu.matlab.tex


==> Figures/NormalPrincipalPressureAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_i/p$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=0^\circ$\end{tabular}}%
\psfrag{s05}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_i/p$\end{tabular}}%
\psfrag{s08}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=6^\circ$\end{tabular}}%
\psfrag{s09}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s11}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_i/p$\end{tabular}}%
\psfrag{s13}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=15^\circ$\end{tabular}}%
\psfrag{s16}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s17}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s18}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s19}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s20}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s21}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{0.5}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{0.5}%
\psfrag{x09}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.6}%
\psfrag{v02}[r][r]{0.7}%
\psfrag{v03}[r][r]{0.8}%
\psfrag{v04}[r][r]{0.9}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{1.1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.3}%
\psfrag{v09}[r][r]{1.4}%
\psfrag{v10}[r][r]{0.6}%
\psfrag{v11}[r][r]{0.7}%
\psfrag{v12}[r][r]{0.8}%
\psfrag{v13}[r][r]{0.9}%
\psfrag{v14}[r][r]{1}%
\psfrag{v15}[r][r]{1.1}%
\psfrag{v16}[r][r]{1.2}%
\psfrag{v17}[r][r]{1.3}%
\psfrag{v18}[r][r]{1.4}%
\psfrag{v19}[r][r]{0.6}%
\psfrag{v20}[r][r]{0.7}%
\psfrag{v21}[r][r]{0.8}%
\psfrag{v22}[r][r]{0.9}%
\psfrag{v23}[r][r]{1}%
\psfrag{v24}[r][r]{1.1}%
\psfrag{v25}[r][r]{1.2}%
\psfrag{v26}[r][r]{1.3}%
\psfrag{v27}[r][r]{1.4}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalPrincipalPressureAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End NormalPrincipalPressureAnisotropy.matlab.tex


==> Figures/NormalStress.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{normal,flow}/\sigma_{flow}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h\approx26$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h\approx7.8$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h\approx17$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h\approx26$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{23}%
\psfrag{x02}[t][t]{23.5}%
\psfrag{x03}[t][t]{24}%
\psfrag{x04}[t][t]{24.5}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{25.5}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{26.5}%
\psfrag{x09}[t][t]{27}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.965}%
\psfrag{v02}[r][r]{0.97}%
\psfrag{v03}[r][r]{0.975}%
\psfrag{v04}[r][r]{0.98}%
\psfrag{v05}[r][r]{0.985}%
%
% Figure:
\resizebox{7cm}{!}{\includegraphics{NormalStress.matlab.eps}}%
\end{psfrags}%
%
% End NormalStress.matlab.tex


==> Figures/NormalStressAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{ii}/p$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{zz}/p$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{xx}/p$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{yy}/p$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{zz}/p$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.8}%
\psfrag{v02}[r][r]{0.85}%
\psfrag{v03}[r][r]{0.9}%
\psfrag{v04}[r][r]{0.95}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{1.05}%
\psfrag{v07}[r][r]{1.1}%
\psfrag{v08}[r][r]{1.15}%
\psfrag{v09}[r][r]{1.2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy.matlab.tex


==> Figures/NormalStressAnisotropy_Fabric.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$F_{xz}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$tr(F)$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$F_{xz}$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.05}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{0.05}%
\psfrag{v04}[r][r]{0.1}%
\psfrag{v05}[r][r]{0.15}%
\psfrag{v06}[r][r]{0.2}%
\psfrag{v07}[r][r]{0.25}%
\psfrag{v08}[r][r]{0.3}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_Fabric.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_Fabric.matlab.tex


==> Figures/NormalStressAnisotropy_FabricAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$F_{zz}/tr(F)$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$F_{xx}/tr(F)$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$F_{yy}/tr(F)$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$F_{zz}/tr(F)$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.8}%
\psfrag{v02}[r][r]{0.85}%
\psfrag{v03}[r][r]{0.9}%
\psfrag{v04}[r][r]{0.95}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{1.05}%
\psfrag{v07}[r][r]{1.1}%
\psfrag{v08}[r][r]{1.15}%
\psfrag{v09}[r][r]{1.2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_FabricAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_FabricAnisotropy.matlab.tex


==> Figures/NormalStressAnisotropy_FabricPrinAngle.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\phi_{F,3}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$-\phi_{F,1}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\phi_{F,3}$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.2}%
\psfrag{x02}[t][t]{0.4}%
\psfrag{x03}[t][t]{0.6}%
\psfrag{x04}[t][t]{0.8}%
\psfrag{x05}[t][t]{1}%
\psfrag{x06}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{40}%
\psfrag{v02}[r][r]{41}%
\psfrag{v03}[r][r]{42}%
\psfrag{v04}[r][r]{43}%
\psfrag{v05}[r][r]{44}%
\psfrag{v06}[r][r]{45}%
\psfrag{v07}[r][r]{46}%
\psfrag{v08}[r][r]{47}%
\psfrag{v09}[r][r]{48}%
\psfrag{v10}[r][r]{49}%
\psfrag{v11}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_FabricPrinAngle.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_FabricPrinAngle.matlab.tex


==> Figures/NormalStressAnisotropy_FabricPrinEVal.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$F_{3}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$F_{1}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$F_{2}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$F_{3}$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.2}%
\psfrag{x02}[t][t]{0.4}%
\psfrag{x03}[t][t]{0.6}%
\psfrag{x04}[t][t]{0.8}%
\psfrag{x05}[t][t]{1}%
\psfrag{x06}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{1.5}%
\psfrag{v04}[r][r]{2}%
\psfrag{v05}[r][r]{2.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_FabricPrinEVal.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_FabricPrinEVal.matlab.tex


==> Figures/NormalStressAnisotropy_SigmaKin.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{kin,xz}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{kin,xx}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{kin,yy}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{kin,zz}$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{kin,xz}$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.01}%
\psfrag{v03}[r][r]{0.02}%
\psfrag{v04}[r][r]{0.03}%
\psfrag{v05}[r][r]{0.04}%
\psfrag{v06}[r][r]{0.05}%
\psfrag{v07}[r][r]{0.06}%
\psfrag{v08}[r][r]{0.07}%
\psfrag{v09}[r][r]{0.08}%
\psfrag{v10}[r][r]{0.09}%
\psfrag{v11}[r][r]{0.1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_SigmaKin.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_SigmaKin.matlab.tex


==> Figures/NormalStressAnisotropy_SigmaKinPrinAngle.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\phi_{kin,2}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\phi_{kin,1}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\phi_{kin,2}$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.2}%
\psfrag{x02}[t][t]{0.4}%
\psfrag{x03}[t][t]{0.6}%
\psfrag{x04}[t][t]{0.8}%
\psfrag{x05}[t][t]{1}%
\psfrag{x06}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{-80}%
\psfrag{v02}[r][r]{-60}%
\psfrag{v03}[r][r]{-40}%
\psfrag{v04}[r][r]{-20}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{20}%
\psfrag{v07}[r][r]{40}%
\psfrag{v08}[r][r]{60}%
\psfrag{v09}[r][r]{80}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_SigmaKinPrinAngle.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_SigmaKinPrinAngle.matlab.tex


==> Figures/NormalStressAnisotropy_SigmaKinPrinEVal.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{kin,3}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{kin,1}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{kin,2}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{kin,3}$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.2}%
\psfrag{x02}[t][t]{0.4}%
\psfrag{x03}[t][t]{0.6}%
\psfrag{x04}[t][t]{0.8}%
\psfrag{x05}[t][t]{1}%
\psfrag{x06}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.01}%
\psfrag{v02}[r][r]{0.02}%
\psfrag{v03}[r][r]{0.03}%
\psfrag{v04}[r][r]{0.04}%
\psfrag{v05}[r][r]{0.05}%
\psfrag{v06}[r][r]{0.06}%
\psfrag{v07}[r][r]{0.07}%
\psfrag{v08}[r][r]{0.08}%
\psfrag{v09}[r][r]{0.09}%
\psfrag{v10}[r][r]{0.1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_SigmaKinPrinEVal.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_SigmaKinPrinEVal.matlab.tex


==> Figures/NormalStressAnisotropy_SigmaNorPrinAngle.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\phi_{normal,3}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$-\phi_{normal,1}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\phi_{normal,3}$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.2}%
\psfrag{x02}[t][t]{0.4}%
\psfrag{x03}[t][t]{0.6}%
\psfrag{x04}[t][t]{0.8}%
\psfrag{x05}[t][t]{1}%
\psfrag{x06}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{40}%
\psfrag{v02}[r][r]{41}%
\psfrag{v03}[r][r]{42}%
\psfrag{v04}[r][r]{43}%
\psfrag{v05}[r][r]{44}%
\psfrag{v06}[r][r]{45}%
\psfrag{v07}[r][r]{46}%
\psfrag{v08}[r][r]{47}%
\psfrag{v09}[r][r]{48}%
\psfrag{v10}[r][r]{49}%
\psfrag{v11}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_SigmaNorPrinAngle.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_SigmaNorPrinAngle.matlab.tex


==> Figures/NormalStressAnisotropy_SigmaNorPrinEVal.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{normal,3}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{normal,1}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{normal,2}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{normal,3}$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.2}%
\psfrag{x02}[t][t]{0.4}%
\psfrag{x03}[t][t]{0.6}%
\psfrag{x04}[t][t]{0.8}%
\psfrag{x05}[t][t]{1}%
\psfrag{x06}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{2}%
\psfrag{v02}[r][r]{4}%
\psfrag{v03}[r][r]{6}%
\psfrag{v04}[r][r]{8}%
\psfrag{v05}[r][r]{10}%
\psfrag{v06}[r][r]{12}%
\psfrag{v07}[r][r]{14}%
\psfrag{v08}[r][r]{16}%
\psfrag{v09}[r][r]{18}%
\psfrag{v10}[r][r]{20}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_SigmaNorPrinEVal.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_SigmaNorPrinEVal.matlab.tex


==> Figures/NormalStressAnisotropy_SigmaNormal.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{normal,xz}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{normal,xx}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{normal,yy}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{normal,zz}$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{normal,xz}$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{-4}%
\psfrag{v02}[r][r]{-2}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{2}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{6}%
\psfrag{v07}[r][r]{8}%
\psfrag{v08}[r][r]{10}%
\psfrag{v09}[r][r]{12}%
\psfrag{v10}[r][r]{14}%
\psfrag{v11}[r][r]{16}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_SigmaNormal.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_SigmaNormal.matlab.tex


==> Figures/NormalStressAnisotropy_SigmaTanPrinAngle.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\phi_{tang,3}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$-\phi_{tang,1}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\phi_{tang,3}$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.2}%
\psfrag{x02}[t][t]{0.4}%
\psfrag{x03}[t][t]{0.6}%
\psfrag{x04}[t][t]{0.8}%
\psfrag{x05}[t][t]{1}%
\psfrag{x06}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{40}%
\psfrag{v02}[r][r]{41}%
\psfrag{v03}[r][r]{42}%
\psfrag{v04}[r][r]{43}%
\psfrag{v05}[r][r]{44}%
\psfrag{v06}[r][r]{45}%
\psfrag{v07}[r][r]{46}%
\psfrag{v08}[r][r]{47}%
\psfrag{v09}[r][r]{48}%
\psfrag{v10}[r][r]{49}%
\psfrag{v11}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_SigmaTanPrinAngle.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_SigmaTanPrinAngle.matlab.tex


==> Figures/NormalStressAnisotropy_SigmaTanPrinEVal.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{tang,3}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{tang,1}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{tang,2}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{tang,3}$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.2}%
\psfrag{x02}[t][t]{0.4}%
\psfrag{x03}[t][t]{0.6}%
\psfrag{x04}[t][t]{0.8}%
\psfrag{x05}[t][t]{1}%
\psfrag{x06}[t][t]{1.2}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.8}%
\psfrag{v02}[r][r]{-0.6}%
\psfrag{v03}[r][r]{-0.4}%
\psfrag{v04}[r][r]{-0.2}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{0.2}%
\psfrag{v07}[r][r]{0.4}%
\psfrag{v08}[r][r]{0.6}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_SigmaTanPrinEVal.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_SigmaTanPrinEVal.matlab.tex


==> Figures/NormalStressAnisotropy_SigmaTangential.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{tang,xz}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{tang,xx}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{tang,yy}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{tang,zz}$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{tang,xz}$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.8}%
\psfrag{v02}[r][r]{-0.6}%
\psfrag{v03}[r][r]{-0.4}%
\psfrag{v04}[r][r]{-0.2}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{0.2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalStressAnisotropy_SigmaTangential.matlab.eps}}%
\end{psfrags}%
%
% End NormalStressAnisotropy_SigmaTangential.matlab.tex


==> Figures/NormalTraceF.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$tr(F)$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=15^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=0^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=6^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=15^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
\psfrag{v06}[r][r]{2.5}%
\psfrag{v07}[r][r]{3}%
\psfrag{v08}[r][r]{3.5}%
\psfrag{v09}[r][r]{4}%
\psfrag{v10}[r][r]{4.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{NormalTraceF.matlab.eps}}%
\end{psfrags}%
%
% End NormalTraceF.matlab.tex


==> Figures/PrincipalStressAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_i/p$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_3/p$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_1/p$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_2/p$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_3/p$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.4}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.4}%
\psfrag{v09}[r][r]{1.6}%
\psfrag{v10}[r][r]{1.8}%
\psfrag{v11}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{PrincipalStressAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End PrincipalStressAnisotropy.matlab.tex


==> Figures/PrincipalStressAnisotropy2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$(\phi_1)_{flow}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=37.5}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=17.5}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=27.5}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=37.5}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{23}%
\psfrag{x02}[t][t]{23.5}%
\psfrag{x03}[t][t]{24}%
\psfrag{x04}[t][t]{24.5}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{25.5}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{26.5}%
\psfrag{x09}[t][t]{27}%
%
% yticklabels:
\psfrag{v01}[r][r]{44.6}%
\psfrag{v02}[r][r]{44.8}%
\psfrag{v03}[r][r]{45}%
\psfrag{v04}[r][r]{45.2}%
\psfrag{v05}[r][r]{45.4}%
\psfrag{v06}[r][r]{45.6}%
\psfrag{v07}[r][r]{45.8}%
\psfrag{v08}[r][r]{46}%
\psfrag{v09}[r][r]{46.2}%
\psfrag{v10}[r][r]{46.4}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{PrincipalStressAnisotropy2.matlab.eps}}%
\end{psfrags}%
%
% End PrincipalStressAnisotropy2.matlab.tex


==> Figures/PrincipalStressEVec.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_1$\end{tabular}}%
\psfrag{s05}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s08}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_2$\end{tabular}}%
\psfrag{s09}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s12}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_3$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{0.5}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{0.5}%
\psfrag{x09}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{43}%
\psfrag{v02}[r][r]{43.5}%
\psfrag{v03}[r][r]{44}%
\psfrag{v04}[r][r]{44.5}%
\psfrag{v05}[r][r]{45}%
\psfrag{v06}[r][r]{45.5}%
\psfrag{v07}[r][r]{46}%
\psfrag{v08}[r][r]{46.5}%
\psfrag{v09}[r][r]{47}%
\psfrag{v10}[r][r]{88}%
\psfrag{v11}[r][r]{88.5}%
\psfrag{v12}[r][r]{89}%
\psfrag{v13}[r][r]{89.5}%
\psfrag{v14}[r][r]{90}%
\psfrag{v15}[r][r]{90.5}%
\psfrag{v16}[r][r]{91}%
\psfrag{v17}[r][r]{91.5}%
\psfrag{v18}[r][r]{92}%
\psfrag{v19}[r][r]{43}%
\psfrag{v20}[r][r]{43.5}%
\psfrag{v21}[r][r]{44}%
\psfrag{v22}[r][r]{44.5}%
\psfrag{v23}[r][r]{45}%
\psfrag{v24}[r][r]{45.5}%
\psfrag{v25}[r][r]{46}%
\psfrag{v26}[r][r]{46.5}%
\psfrag{v27}[r][r]{47}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{PrincipalStressEVec.matlab.eps}}%
\end{psfrags}%
%
% End PrincipalStressEVec.matlab.tex


==> Figures/PrincipalStressEVecOverTime.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t_{max}$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\bar\phi_1$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2000}%
\psfrag{x02}[t][t]{2500}%
\psfrag{x03}[t][t]{3000}%
\psfrag{x04}[t][t]{3500}%
\psfrag{x05}[t][t]{4000}%
\psfrag{x06}[t][t]{4500}%
\psfrag{x07}[t][t]{5000}%
\psfrag{x08}[t][t]{5500}%
\psfrag{x09}[t][t]{6000}%
\psfrag{x10}[t][t]{6500}%
\psfrag{x11}[t][t]{7000}%
%
% yticklabels:
\psfrag{v01}[r][r]{45}%
\psfrag{v02}[r][r]{45.1}%
\psfrag{v03}[r][r]{45.2}%
\psfrag{v04}[r][r]{45.3}%
\psfrag{v05}[r][r]{45.4}%
\psfrag{v06}[r][r]{45.5}%
\psfrag{v07}[r][r]{45.6}%
\psfrag{v08}[r][r]{45.7}%
\psfrag{v09}[r][r]{45.8}%
\psfrag{v10}[r][r]{45.9}%
\psfrag{v11}[r][r]{46}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{PrincipalStressEVecOverTime.matlab.eps}}%
\end{psfrags}%
%
% End PrincipalStressEVecOverTime.matlab.tex


==> Figures/PrincipalStressEVecW.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_1$\end{tabular}}%
\psfrag{s05}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s08}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_2$\end{tabular}}%
\psfrag{s09}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s12}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_3$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{0.5}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{0.5}%
\psfrag{x09}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{40}%
\psfrag{v02}[r][r]{41}%
\psfrag{v03}[r][r]{42}%
\psfrag{v04}[r][r]{43}%
\psfrag{v05}[r][r]{44}%
\psfrag{v06}[r][r]{45}%
\psfrag{v07}[r][r]{46}%
\psfrag{v08}[r][r]{47}%
\psfrag{v09}[r][r]{48}%
\psfrag{v10}[r][r]{49}%
\psfrag{v11}[r][r]{50}%
\psfrag{v12}[r][r]{80}%
\psfrag{v13}[r][r]{82}%
\psfrag{v14}[r][r]{84}%
\psfrag{v15}[r][r]{86}%
\psfrag{v16}[r][r]{88}%
\psfrag{v17}[r][r]{90}%
\psfrag{v18}[r][r]{92}%
\psfrag{v19}[r][r]{94}%
\psfrag{v20}[r][r]{96}%
\psfrag{v21}[r][r]{98}%
\psfrag{v22}[r][r]{100}%
\psfrag{v23}[r][r]{40}%
\psfrag{v24}[r][r]{41}%
\psfrag{v25}[r][r]{42}%
\psfrag{v26}[r][r]{43}%
\psfrag{v27}[r][r]{44}%
\psfrag{v28}[r][r]{45}%
\psfrag{v29}[r][r]{46}%
\psfrag{v30}[r][r]{47}%
\psfrag{v31}[r][r]{48}%
\psfrag{v32}[r][r]{49}%
\psfrag{v33}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{PrincipalStressEVecW.matlab.eps}}%
\end{psfrags}%
%
% End PrincipalStressEVecW.matlab.tex


==> Figures/W.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=2.5$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.05$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.1$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.2$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.3$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.4$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.5$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=1.5$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=2.5$}%
\psfrag{s15}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s16}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.4}%
\psfrag{v02}[r][r]{0.42}%
\psfrag{v03}[r][r]{0.44}%
\psfrag{v04}[r][r]{0.46}%
\psfrag{v05}[r][r]{0.48}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.52}%
\psfrag{v08}[r][r]{0.54}%
\psfrag{v09}[r][r]{0.56}%
\psfrag{v10}[r][r]{0.58}%
\psfrag{v11}[r][r]{0.6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{W.matlab.eps}}%
\end{psfrags}%
%
% End W.matlab.tex


==> Figures/WFlowVelocity.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{1.5}%
\psfrag{v04}[r][r]{2}%
\psfrag{v05}[r][r]{2.5}%
\psfrag{v06}[r][r]{3}%
\psfrag{v07}[r][r]{3.5}%
\psfrag{v08}[r][r]{4}%
\psfrag{v09}[r][r]{4.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{WFlowVelocity.matlab.eps}}%
\end{psfrags}%
%
% End WFlowVelocity.matlab.tex


==> Figures/WKineticStressXX.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{kin\ xx}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{WKineticStressXX.matlab.eps}}%
\end{psfrags}%
%
% End WKineticStressXX.matlab.tex


==> Figures/WKineticStressZZ.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{kin\ zz}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.01}%
\psfrag{v03}[r][r]{0.02}%
\psfrag{v04}[r][r]{0.03}%
\psfrag{v05}[r][r]{0.04}%
\psfrag{v06}[r][r]{0.05}%
\psfrag{v07}[r][r]{0.06}%
\psfrag{v08}[r][r]{0.07}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{WKineticStressZZ.matlab.eps}}%
\end{psfrags}%
%
% End WKineticStressZZ.matlab.tex


==> Figures/WLegend_.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.00625$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=2.5$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=2.25$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=2$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=1.5$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=1.25$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=1$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.9$}%
\psfrag{s15}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.8$}%
\psfrag{s16}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.7$}%
\psfrag{s17}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.6$}%
\psfrag{s18}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.5$}%
\psfrag{s19}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.4$}%
\psfrag{s20}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.3$}%
\psfrag{s21}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.2$}%
\psfrag{s22}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s23}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s25}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.1$}%
\psfrag{s27}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.05$}%
\psfrag{s29}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.025$}%
\psfrag{s30}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.0125$}%
\psfrag{s31}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.00625$}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{1}%
%
% Figure:
\resizebox{10cm}{!}{\includegraphics{WLegend_.matlab.eps}}%
\end{psfrags}%
%
% End WLegend_.matlab.tex


==> Figures/WMu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}/\sigma_{zz}$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.45}%
\psfrag{v02}[r][r]{0.46}%
\psfrag{v03}[r][r]{0.47}%
\psfrag{v04}[r][r]{0.48}%
\psfrag{v05}[r][r]{0.49}%
\psfrag{v06}[r][r]{0.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{WMu.matlab.eps}}%
\end{psfrags}%
%
% End WMu.matlab.tex


==> Figures/WNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{WNu.matlab.eps}}%
\end{psfrags}%
%
% End WNu.matlab.tex


==> Figures/Wnorm.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$w$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\|\phi\|_w$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\|\nu\|_w$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\|v_x\|_w$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\|s_D\|_w$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\|p\|_w$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\|\phi\|_w$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.5}%
\psfrag{x02}[t][t]{1}%
\psfrag{x03}[t][t]{1.5}%
\psfrag{x04}[t][t]{2}%
\psfrag{x05}[t][t]{2.5}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{-2}$}%
\psfrag{v02}[r][r]{$10^{-1}$}%
\psfrag{v03}[r][r]{$10^{0}$}%
\psfrag{v04}[r][r]{$10^{1}$}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{Wnorm.matlab.eps}}%
\end{psfrags}%
%
% End Wnorm.matlab.tex


==> Figures/XNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$L_x=30, L_y=15$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$L_x=10, L_y=5$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$L_x=20, L_y=10$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$L_x=30, L_y=15$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.55}%
\psfrag{v02}[r][r]{0.56}%
\psfrag{v03}[r][r]{0.57}%
\psfrag{v04}[r][r]{0.58}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{XNu.matlab.eps}}%
\end{psfrags}%
%
% End XNu.matlab.tex


==> Figures/XV.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$L_x=30, L_y=15$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$L_x=10, L_y=5$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$L_x=20, L_y=10$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$L_x=30, L_y=15$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{1.5}%
\psfrag{v04}[r][r]{2}%
\psfrag{v05}[r][r]{2.5}%
\psfrag{v06}[r][r]{3}%
\psfrag{v07}[r][r]{3.5}%
\psfrag{v08}[r][r]{4}%
\psfrag{v09}[r][r]{4.5}%
\psfrag{v10}[r][r]{5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{XV.matlab.eps}}%
\end{psfrags}%
%
% End XV.matlab.tex


==> Figures/bprNu2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.75$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1.25$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1.5$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{bprNu2.matlab.eps}}%
\end{psfrags}%
%
% End bprNu2.matlab.tex


==> Figures/bprNuOld.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.5$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.25$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.5$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{bprNu.matlab.eps}}%
\end{psfrags}%
%
% End bprNu.matlab.tex


==> Figures/bprPrincipalStress.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s09}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s10}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=2.6e+02, a=31$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=16, a=20$}%
\psfrag{s16}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=16, a=20$}%
\psfrag{s17}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=16, a=21$}%
\psfrag{s18}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=17, a=21$}%
\psfrag{s19}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=17, a=22$}%
\psfrag{s20}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=17, a=22$}%
\psfrag{s21}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=17, a=23$}%
\psfrag{s22}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=17, a=25$}%
\psfrag{s23}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=18, a=27$}%
\psfrag{s24}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=21, a=30$}%
\psfrag{s25}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h=2.6e+02, a=31$}%
\psfrag{s26}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s27}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
\psfrag{x12}[t][t]{0}%
\psfrag{x13}[t][t]{5}%
\psfrag{x14}[t][t]{10}%
\psfrag{x15}[t][t]{15}%
\psfrag{x16}[t][t]{20}%
\psfrag{x17}[t][t]{25}%
\psfrag{x18}[t][t]{0}%
\psfrag{x19}[t][t]{5}%
\psfrag{x20}[t][t]{10}%
\psfrag{x21}[t][t]{15}%
\psfrag{x22}[t][t]{20}%
\psfrag{x23}[t][t]{25}%
%
% yticklabels:
\psfrag{v01}[r][r]{20}%
\psfrag{v02}[r][r]{40}%
\psfrag{v03}[r][r]{60}%
\psfrag{v04}[r][r]{80}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{50}%
\psfrag{v07}[r][r]{100}%
\psfrag{v08}[r][r]{0}%
\psfrag{v09}[r][r]{50}%
\psfrag{v10}[r][r]{100}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{bprPrincipalStress.matlab.eps}}%
\end{psfrags}%
%
% End bprPrincipalStress.matlab.tex


==> Figures/bprVelocityX2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.75$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1.25$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1.5$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{1.5}%
\psfrag{v04}[r][r]{2}%
\psfrag{v05}[r][r]{2.5}%
\psfrag{v06}[r][r]{3}%
\psfrag{v07}[r][r]{3.5}%
\psfrag{v08}[r][r]{4}%
\psfrag{v09}[r][r]{4.5}%
\psfrag{v10}[r][r]{5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{bprVelocityX2.matlab.eps}}%
\end{psfrags}%
%
% End bprVelocityX2.matlab.tex


==> Figures/bprVelocityXold.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.5$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.25$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=0.5$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{5}%
\psfrag{v02}[r][r]{10}%
\psfrag{v03}[r][r]{15}%
\psfrag{v04}[r][r]{20}%
\psfrag{v05}[r][r]{25}%
\psfrag{v06}[r][r]{30}%
\psfrag{v07}[r][r]{35}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{bprVelocityX.matlab.eps}}%
\end{psfrags}%
%
% End bprVelocityX.matlab.tex


==> Figures/domainNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rho$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=30, l_y=15$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=10, l_y=5$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=20, l_y=10$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=30, l_y=15$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{domainNu.matlab.eps}}%
\end{psfrags}%
%
% End domainNu.matlab.tex


==> Figures/domainVelocityX.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=30, l_y=15$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=10, l_y=5$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=20, l_y=10$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=30, l_y=15$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{domainVelocityX.matlab.eps}}%
\end{psfrags}%
%
% End domainVelocityX.matlab.tex


==> Figures/dxNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rho$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=30, l_y=10$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=10, l_y=10$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=20, l_y=10$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=30, l_y=10$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{dxNu.matlab.eps}}%
\end{psfrags}%
%
% End dxNu.matlab.tex


==> Figures/dxVelocityX.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=30, l_y=10$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=10, l_y=10$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=20, l_y=10$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$l_x=30, l_y=10$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{dxVelocityX.matlab.eps}}%
\end{psfrags}%
%
% End dxVelocityX.matlab.tex


==> Figures/ene.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1386,660){\makebox(0,0)[r]{\strut{} 1e-25}}%
      \put(1386,1280){\makebox(0,0)[r]{\strut{} 1e-20}}%
      \put(1386,1900){\makebox(0,0)[r]{\strut{} 1e-15}}%
      \put(1386,2520){\makebox(0,0)[r]{\strut{} 1e-10}}%
      \put(1386,3140){\makebox(0,0)[r]{\strut{} 1e-05}}%
      \put(1386,3760){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1386,4380){\makebox(0,0)[r]{\strut{} 100000}}%
      \put(1518,440){\makebox(0,0){\strut{} 0}}%
      \put(2049,440){\makebox(0,0){\strut{} 200}}%
      \put(2580,440){\makebox(0,0){\strut{} 400}}%
      \put(3110,440){\makebox(0,0){\strut{} 600}}%
      \put(3641,440){\makebox(0,0){\strut{} 800}}%
      \put(4172,440){\makebox(0,0){\strut{} 1000}}%
      \put(4703,440){\makebox(0,0){\strut{} 1200}}%
      \put(5234,440){\makebox(0,0){\strut{} 1400}}%
      \put(5764,440){\makebox(0,0){\strut{} 1600}}%
      \put(6295,440){\makebox(0,0){\strut{} 1800}}%
      \put(6826,440){\makebox(0,0){\strut{} 2000}}%
      \put(220,2520){\rotatebox{90}{\makebox(0,0){\strut{}Ekin}}}%
      \put(4172,110){\makebox(0,0){\strut{}t}}%
      \put(4172,4710){\makebox(0,0){\strut{}Kinetic energy for height h=20d, varying chute angle and timestep}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5839,4207){\makebox(0,0)[r]{\strut{}23 deg h=5}}%
      \csname LTb\endcsname%
      \put(5839,3987){\makebox(0,0)[r]{\strut{}23.5 deg h=5}}%
      \csname LTb\endcsname%
      \put(5839,3767){\makebox(0,0)[r]{\strut{}24 deg h=5}}%
      \csname LTb\endcsname%
      \put(5839,3547){\makebox(0,0)[r]{\strut{}24.5 deg h=5}}%
      \csname LTb\endcsname%
      \put(5839,3327){\makebox(0,0)[r]{\strut{}25 deg h=5}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1386,660){\makebox(0,0)[r]{\strut{} 1e-25}}%
      \put(1386,1280){\makebox(0,0)[r]{\strut{} 1e-20}}%
      \put(1386,1900){\makebox(0,0)[r]{\strut{} 1e-15}}%
      \put(1386,2520){\makebox(0,0)[r]{\strut{} 1e-10}}%
      \put(1386,3140){\makebox(0,0)[r]{\strut{} 1e-05}}%
      \put(1386,3760){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1386,4380){\makebox(0,0)[r]{\strut{} 100000}}%
      \put(1518,440){\makebox(0,0){\strut{} 0}}%
      \put(2049,440){\makebox(0,0){\strut{} 200}}%
      \put(2580,440){\makebox(0,0){\strut{} 400}}%
      \put(3110,440){\makebox(0,0){\strut{} 600}}%
      \put(3641,440){\makebox(0,0){\strut{} 800}}%
      \put(4172,440){\makebox(0,0){\strut{} 1000}}%
      \put(4703,440){\makebox(0,0){\strut{} 1200}}%
      \put(5234,440){\makebox(0,0){\strut{} 1400}}%
      \put(5764,440){\makebox(0,0){\strut{} 1600}}%
      \put(6295,440){\makebox(0,0){\strut{} 1800}}%
      \put(6826,440){\makebox(0,0){\strut{} 2000}}%
      \put(220,2520){\rotatebox{90}{\makebox(0,0){\strut{}Ekin}}}%
      \put(4172,110){\makebox(0,0){\strut{}t}}%
      \put(4172,4710){\makebox(0,0){\strut{}Kinetic energy for height h=20d, varying chute angle and timestep}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5839,4207){\makebox(0,0)[r]{\strut{}21 deg h=10}}%
      \csname LTb\endcsname%
      \put(5839,3987){\makebox(0,0)[r]{\strut{}21.5 deg h=10}}%
      \csname LTb\endcsname%
      \put(5839,3767){\makebox(0,0)[r]{\strut{}22 deg h=10}}%
      \csname LTb\endcsname%
      \put(5839,3547){\makebox(0,0)[r]{\strut{}22.5 deg h=10}}%
      \csname LTb\endcsname%
      \put(5839,3327){\makebox(0,0)[r]{\strut{}23 deg h=10}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1386,660){\makebox(0,0)[r]{\strut{} 1e-10}}%
      \put(1386,1280){\makebox(0,0)[r]{\strut{} 1e-08}}%
      \put(1386,1900){\makebox(0,0)[r]{\strut{} 1e-06}}%
      \put(1386,2520){\makebox(0,0)[r]{\strut{} 0.0001}}%
      \put(1386,3140){\makebox(0,0)[r]{\strut{} 0.01}}%
      \put(1386,3760){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1386,4380){\makebox(0,0)[r]{\strut{} 100}}%
      \put(1518,440){\makebox(0,0){\strut{} 0}}%
      \put(2108,440){\makebox(0,0){\strut{} 100}}%
      \put(2698,440){\makebox(0,0){\strut{} 200}}%
      \put(3287,440){\makebox(0,0){\strut{} 300}}%
      \put(3877,440){\makebox(0,0){\strut{} 400}}%
      \put(4467,440){\makebox(0,0){\strut{} 500}}%
      \put(5057,440){\makebox(0,0){\strut{} 600}}%
      \put(5646,440){\makebox(0,0){\strut{} 700}}%
      \put(6236,440){\makebox(0,0){\strut{} 800}}%
      \put(6826,440){\makebox(0,0){\strut{} 900}}%
      \put(220,2520){\rotatebox{90}{\makebox(0,0){\strut{}Ekin}}}%
      \put(4172,110){\makebox(0,0){\strut{}t}}%
      \put(4172,4710){\makebox(0,0){\strut{}Kinetic energy for height h=20d, varying chute angle and timestep}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5839,4207){\makebox(0,0)[r]{\strut{}20 deg h=20}}%
      \csname LTb\endcsname%
      \put(5839,3987){\makebox(0,0)[r]{\strut{}20.5 deg h=20}}%
      \csname LTb\endcsname%
      \put(5839,3767){\makebox(0,0)[r]{\strut{}21 deg h=20}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1386,660){\makebox(0,0)[r]{\strut{} 1e-08}}%
      \put(1386,1073){\makebox(0,0)[r]{\strut{} 1e-07}}%
      \put(1386,1487){\makebox(0,0)[r]{\strut{} 1e-06}}%
      \put(1386,1900){\makebox(0,0)[r]{\strut{} 1e-05}}%
      \put(1386,2313){\makebox(0,0)[r]{\strut{} 0.0001}}%
      \put(1386,2727){\makebox(0,0)[r]{\strut{} 0.001}}%
      \put(1386,3140){\makebox(0,0)[r]{\strut{} 0.01}}%
      \put(1386,3553){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1386,3967){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1386,4380){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1518,440){\makebox(0,0){\strut{} 0}}%
      \put(2049,440){\makebox(0,0){\strut{} 50}}%
      \put(2580,440){\makebox(0,0){\strut{} 100}}%
      \put(3110,440){\makebox(0,0){\strut{} 150}}%
      \put(3641,440){\makebox(0,0){\strut{} 200}}%
      \put(4172,440){\makebox(0,0){\strut{} 250}}%
      \put(4703,440){\makebox(0,0){\strut{} 300}}%
      \put(5234,440){\makebox(0,0){\strut{} 350}}%
      \put(5764,440){\makebox(0,0){\strut{} 400}}%
      \put(6295,440){\makebox(0,0){\strut{} 450}}%
      \put(6826,440){\makebox(0,0){\strut{} 500}}%
      \put(220,2520){\rotatebox{90}{\makebox(0,0){\strut{}Ekin}}}%
      \put(4172,110){\makebox(0,0){\strut{}t}}%
      \put(4172,4710){\makebox(0,0){\strut{}Kinetic energy for height h=20d, varying chute angle and timestep}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5839,4207){\makebox(0,0)[r]{\strut{}19 deg h=30}}%
      \csname LTb\endcsname%
      \put(5839,3987){\makebox(0,0)[r]{\strut{}19.5 deg h=30}}%
      \csname LTb\endcsname%
      \put(5839,3767){\makebox(0,0)[r]{\strut{}20 deg h=30}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1386,660){\makebox(0,0)[r]{\strut{} 1e-08}}%
      \put(1386,1032){\makebox(0,0)[r]{\strut{} 1e-07}}%
      \put(1386,1404){\makebox(0,0)[r]{\strut{} 1e-06}}%
      \put(1386,1776){\makebox(0,0)[r]{\strut{} 1e-05}}%
      \put(1386,2148){\makebox(0,0)[r]{\strut{} 0.0001}}%
      \put(1386,2520){\makebox(0,0)[r]{\strut{} 0.001}}%
      \put(1386,2892){\makebox(0,0)[r]{\strut{} 0.01}}%
      \put(1386,3264){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1386,3636){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1386,4008){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1386,4380){\makebox(0,0)[r]{\strut{} 100}}%
      \put(1518,440){\makebox(0,0){\strut{} 0}}%
      \put(2182,440){\makebox(0,0){\strut{} 50}}%
      \put(2845,440){\makebox(0,0){\strut{} 100}}%
      \put(3509,440){\makebox(0,0){\strut{} 150}}%
      \put(4172,440){\makebox(0,0){\strut{} 200}}%
      \put(4836,440){\makebox(0,0){\strut{} 250}}%
      \put(5499,440){\makebox(0,0){\strut{} 300}}%
      \put(6163,440){\makebox(0,0){\strut{} 350}}%
      \put(6826,440){\makebox(0,0){\strut{} 400}}%
      \put(220,2520){\rotatebox{90}{\makebox(0,0){\strut{}Ekin}}}%
      \put(4172,110){\makebox(0,0){\strut{}t}}%
      \put(4172,4710){\makebox(0,0){\strut{}Kinetic energy for height h=20d, varying chute angle and timestep}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5839,4207){\makebox(0,0)[r]{\strut{}19 deg h=40}}%
      \csname LTb\endcsname%
      \put(5839,3987){\makebox(0,0)[r]{\strut{}19.5 deg h=40}}%
      \csname LTb\endcsname%
      \put(5839,3767){\makebox(0,0)[r]{\strut{}20 deg h=40}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ene}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/ene_h10.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4534.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1562,660){\makebox(0,0)[r]{\strut{}$10^{-18}$}}%
      \put(1562,885){\makebox(0,0)[r]{\strut{}$10^{-16}$}}%
      \put(1562,1110){\makebox(0,0)[r]{\strut{}$10^{-14}$}}%
      \put(1562,1335){\makebox(0,0)[r]{\strut{}$10^{-12}$}}%
      \put(1562,1560){\makebox(0,0)[r]{\strut{}$10^{-10}$}}%
      \put(1562,1785){\makebox(0,0)[r]{\strut{}$10^{-8}$}}%
      \put(1562,2011){\makebox(0,0)[r]{\strut{}$10^{-6}$}}%
      \put(1562,2236){\makebox(0,0)[r]{\strut{}$10^{-4}$}}%
      \put(1562,2461){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(1562,2686){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(1562,2911){\makebox(0,0)[r]{\strut{}$10^{2}$}}%
      \put(1562,3136){\makebox(0,0)[r]{\strut{}$10^{4}$}}%
      \put(1694,440){\makebox(0,0){\strut{} 0}}%
      \put(1968,440){\makebox(0,0){\strut{} 100}}%
      \put(2242,440){\makebox(0,0){\strut{} 200}}%
      \put(2516,440){\makebox(0,0){\strut{} 300}}%
      \put(2790,440){\makebox(0,0){\strut{} 400}}%
      \put(3064,440){\makebox(0,0){\strut{} 500}}%
      \put(3338,440){\makebox(0,0){\strut{} 600}}%
      \put(3612,440){\makebox(0,0){\strut{} 700}}%
      \put(3886,440){\makebox(0,0){\strut{} 800}}%
      \put(4160,440){\makebox(0,0){\strut{} 900}}%
      \put(924,1898){\rotatebox{90}{\makebox(0,0){\strut{}$E_{kin}/E_{elastic}$}}}%
      \put(2927,110){\makebox(0,0){\strut{}t}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3173,2963){\makebox(0,0)[r]{\strut{}$21^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2743){\makebox(0,0)[r]{\strut{}$22^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2523){\makebox(0,0)[r]{\strut{}$23^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2303){\makebox(0,0)[r]{\strut{}$24^{\circ}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ene_h10}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/ene_h20.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4534.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1562,660){\makebox(0,0)[r]{\strut{}$10^{-10}$}}%
      \put(1562,1014){\makebox(0,0)[r]{\strut{}$10^{-8}$}}%
      \put(1562,1367){\makebox(0,0)[r]{\strut{}$10^{-6}$}}%
      \put(1562,1721){\makebox(0,0)[r]{\strut{}$10^{-4}$}}%
      \put(1562,2075){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(1562,2429){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(1562,2782){\makebox(0,0)[r]{\strut{}$10^{2}$}}%
      \put(1562,3136){\makebox(0,0)[r]{\strut{}$10^{4}$}}%
      \put(1694,440){\makebox(0,0){\strut{} 0}}%
      \put(2046,440){\makebox(0,0){\strut{} 50}}%
      \put(2399,440){\makebox(0,0){\strut{} 100}}%
      \put(2751,440){\makebox(0,0){\strut{} 150}}%
      \put(3103,440){\makebox(0,0){\strut{} 200}}%
      \put(3455,440){\makebox(0,0){\strut{} 250}}%
      \put(3808,440){\makebox(0,0){\strut{} 300}}%
      \put(4160,440){\makebox(0,0){\strut{} 350}}%
      \put(924,1898){\rotatebox{90}{\makebox(0,0){\strut{}$E_{kin}/E_{elastic}$}}}%
      \put(2927,110){\makebox(0,0){\strut{}t}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3173,2963){\makebox(0,0)[r]{\strut{}$20^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2743){\makebox(0,0)[r]{\strut{}$20.5^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2523){\makebox(0,0)[r]{\strut{}$21^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2303){\makebox(0,0)[r]{\strut{}$21.5^{\circ}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ene_h20}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/ene_h30.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4534.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1430,660){\makebox(0,0)[r]{\strut{}$10^{-8}$}}%
      \put(1430,1073){\makebox(0,0)[r]{\strut{}$10^{-6}$}}%
      \put(1430,1485){\makebox(0,0)[r]{\strut{}$10^{-4}$}}%
      \put(1430,1898){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(1430,2311){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(1430,2723){\makebox(0,0)[r]{\strut{}$10^{2}$}}%
      \put(1430,3136){\makebox(0,0)[r]{\strut{}$10^{4}$}}%
      \put(1562,440){\makebox(0,0){\strut{} 0}}%
      \put(1851,440){\makebox(0,0){\strut{} 20}}%
      \put(2139,440){\makebox(0,0){\strut{} 40}}%
      \put(2428,440){\makebox(0,0){\strut{} 60}}%
      \put(2717,440){\makebox(0,0){\strut{} 80}}%
      \put(3005,440){\makebox(0,0){\strut{} 100}}%
      \put(3294,440){\makebox(0,0){\strut{} 120}}%
      \put(3583,440){\makebox(0,0){\strut{} 140}}%
      \put(3871,440){\makebox(0,0){\strut{} 160}}%
      \put(4160,440){\makebox(0,0){\strut{} 180}}%
      \put(924,1898){\rotatebox{90}{\makebox(0,0){\strut{}$E_{kin}/E_{elastic}$}}}%
      \put(2861,110){\makebox(0,0){\strut{}t}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3173,2963){\makebox(0,0)[r]{\strut{}$19^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2743){\makebox(0,0)[r]{\strut{}$19.5^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2523){\makebox(0,0)[r]{\strut{}$20^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2303){\makebox(0,0)[r]{\strut{}$20.5^{\circ}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ene_h30}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/ene_h40.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4534.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1430,660){\makebox(0,0)[r]{\strut{}$10^{-6}$}}%
      \put(1430,908){\makebox(0,0)[r]{\strut{}$10^{-5}$}}%
      \put(1430,1155){\makebox(0,0)[r]{\strut{}$10^{-4}$}}%
      \put(1430,1403){\makebox(0,0)[r]{\strut{}$10^{-3}$}}%
      \put(1430,1650){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(1430,1898){\makebox(0,0)[r]{\strut{}$10^{-1}$}}%
      \put(1430,2146){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(1430,2393){\makebox(0,0)[r]{\strut{}$10^{1}$}}%
      \put(1430,2641){\makebox(0,0)[r]{\strut{}$10^{2}$}}%
      \put(1430,2888){\makebox(0,0)[r]{\strut{}$10^{3}$}}%
      \put(1430,3136){\makebox(0,0)[r]{\strut{}$10^{4}$}}%
      \put(1562,440){\makebox(0,0){\strut{} 0}}%
      \put(1822,440){\makebox(0,0){\strut{} 10}}%
      \put(2082,440){\makebox(0,0){\strut{} 20}}%
      \put(2341,440){\makebox(0,0){\strut{} 30}}%
      \put(2601,440){\makebox(0,0){\strut{} 40}}%
      \put(2861,440){\makebox(0,0){\strut{} 50}}%
      \put(3121,440){\makebox(0,0){\strut{} 60}}%
      \put(3381,440){\makebox(0,0){\strut{} 70}}%
      \put(3640,440){\makebox(0,0){\strut{} 80}}%
      \put(3900,440){\makebox(0,0){\strut{} 90}}%
      \put(4160,440){\makebox(0,0){\strut{} 100}}%
      \put(924,1898){\rotatebox{90}{\makebox(0,0){\strut{}$E_{kin}/E_{elastic}$}}}%
      \put(2861,110){\makebox(0,0){\strut{}t}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3173,2963){\makebox(0,0)[r]{\strut{}$19^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2743){\makebox(0,0)[r]{\strut{}$19.5^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2523){\makebox(0,0)[r]{\strut{}$20^{\circ}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ene_h40}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/ene_h5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4534.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1562,660){\makebox(0,0)[r]{\strut{}$10^{-20}$}}%
      \put(1562,1155){\makebox(0,0)[r]{\strut{}$10^{-15}$}}%
      \put(1562,1650){\makebox(0,0)[r]{\strut{}$10^{-10}$}}%
      \put(1562,2146){\makebox(0,0)[r]{\strut{}$10^{-5}$}}%
      \put(1562,2641){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(1562,3136){\makebox(0,0)[r]{\strut{}$10^{5}$}}%
      \put(1694,440){\makebox(0,0){\strut{} 0}}%
      \put(1968,440){\makebox(0,0){\strut{} 200}}%
      \put(2242,440){\makebox(0,0){\strut{} 400}}%
      \put(2516,440){\makebox(0,0){\strut{} 600}}%
      \put(2790,440){\makebox(0,0){\strut{} 800}}%
      \put(3064,440){\makebox(0,0){\strut{} 1000}}%
      \put(3338,440){\makebox(0,0){\strut{} 1200}}%
      \put(3612,440){\makebox(0,0){\strut{} 1400}}%
      \put(3886,440){\makebox(0,0){\strut{} 1600}}%
      \put(4160,440){\makebox(0,0){\strut{} 1800}}%
      \put(924,1898){\rotatebox{90}{\makebox(0,0){\strut{}$E_{kin}/E_{elastic}$}}}%
      \put(2927,110){\makebox(0,0){\strut{}t}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3173,2963){\makebox(0,0)[r]{\strut{}$23^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2743){\makebox(0,0)[r]{\strut{}$24^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2523){\makebox(0,0)[r]{\strut{}$25^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2303){\makebox(0,0)[r]{\strut{}$26^{\circ}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ene_h5}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/ene_h60.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4534.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1430,660){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(1430,1073){\makebox(0,0)[r]{\strut{}$10^{-1}$}}%
      \put(1430,1485){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(1430,1898){\makebox(0,0)[r]{\strut{}$10^{1}$}}%
      \put(1430,2311){\makebox(0,0)[r]{\strut{}$10^{2}$}}%
      \put(1430,2723){\makebox(0,0)[r]{\strut{}$10^{3}$}}%
      \put(1430,3136){\makebox(0,0)[r]{\strut{}$10^{4}$}}%
      \put(1562,440){\makebox(0,0){\strut{} 0}}%
      \put(1798,440){\makebox(0,0){\strut{} 5}}%
      \put(2034,440){\makebox(0,0){\strut{} 10}}%
      \put(2271,440){\makebox(0,0){\strut{} 15}}%
      \put(2507,440){\makebox(0,0){\strut{} 20}}%
      \put(2743,440){\makebox(0,0){\strut{} 25}}%
      \put(2979,440){\makebox(0,0){\strut{} 30}}%
      \put(3215,440){\makebox(0,0){\strut{} 35}}%
      \put(3451,440){\makebox(0,0){\strut{} 40}}%
      \put(3688,440){\makebox(0,0){\strut{} 45}}%
      \put(3924,440){\makebox(0,0){\strut{} 50}}%
      \put(4160,440){\makebox(0,0){\strut{} 55}}%
      \put(924,1898){\rotatebox{90}{\makebox(0,0){\strut{}$E_{kin}/E_{elastic}$}}}%
      \put(2861,110){\makebox(0,0){\strut{}t}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3173,2963){\makebox(0,0)[r]{\strut{}$18^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2743){\makebox(0,0)[r]{\strut{}$18.5^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2523){\makebox(0,0)[r]{\strut{}$19^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2303){\makebox(0,0)[r]{\strut{}$19.5^{\circ}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ene_h60}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/ene_h80.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4534.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1298,660){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(1298,1279){\makebox(0,0)[r]{\strut{}$10^{1}$}}%
      \put(1298,1898){\makebox(0,0)[r]{\strut{}$10^{2}$}}%
      \put(1298,2517){\makebox(0,0)[r]{\strut{}$10^{3}$}}%
      \put(1298,3136){\makebox(0,0)[r]{\strut{}$10^{4}$}}%
      \put(1430,440){\makebox(0,0){\strut{} 0}}%
      \put(1885,440){\makebox(0,0){\strut{} 5}}%
      \put(2340,440){\makebox(0,0){\strut{} 10}}%
      \put(2795,440){\makebox(0,0){\strut{} 15}}%
      \put(3250,440){\makebox(0,0){\strut{} 20}}%
      \put(3705,440){\makebox(0,0){\strut{} 25}}%
      \put(4160,440){\makebox(0,0){\strut{} 30}}%
      \put(924,1898){\rotatebox{90}{\makebox(0,0){\strut{}$E_{kin}/E_{elastic}$}}}%
      \put(2795,110){\makebox(0,0){\strut{}t}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3173,2963){\makebox(0,0)[r]{\strut{}$18^{\circ}$}}%
      \csname LTb\endcsname%
      \put(3173,2743){\makebox(0,0)[r]{\strut{}$19^{\circ}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ene_h80}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/fstatVsTav_KineticStress.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}KineticStressXX\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}KineticStressXY\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}KineticStressXZ\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}KineticStressYY\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}KineticStressYZ\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}KineticStressZZ\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{20}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{10}%
\psfrag{x09}[t][t]{20}%
\psfrag{x10}[t][t]{0}%
\psfrag{x11}[t][t]{10}%
\psfrag{x12}[t][t]{20}%
\psfrag{x13}[t][t]{0}%
\psfrag{x14}[t][t]{10}%
\psfrag{x15}[t][t]{20}%
\psfrag{x16}[t][t]{0}%
\psfrag{x17}[t][t]{10}%
\psfrag{x18}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.05}%
\psfrag{v03}[r][r]{-5}%
\psfrag{v04}[r][r]{0}%
\psfrag{v05}[r][r]{5}%
\psfrag{v06}[r][r]{10}%
\psfrag{v07}[r][r]{0}%
\psfrag{v08}[r][r]{0.05}%
\psfrag{v09}[r][r]{-8}%
\psfrag{v10}[r][r]{-6}%
\psfrag{v11}[r][r]{-4}%
\psfrag{v12}[r][r]{-2}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{-1}%
\psfrag{v15}[r][r]{0}%
\psfrag{v16}[r][r]{1}%
\psfrag{v17}[r][r]{0}%
\psfrag{v18}[r][r]{0.02}%
\psfrag{v19}[r][r]{0.04}%
\psfrag{v20}[r][r]{0.06}%
%
% Figure:
\resizebox{16cm}{!}{\includegraphics{fstatVsTav_KineticStress.matlab.eps}}%
\end{psfrags}%
%
% End fstatVsTav_KineticStress.matlab.tex


==> Figures/fstatVsTav_NormalStress.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}NormalStressXX\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}NormalStressXY\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}NormalStressXZ\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}NormalStressYY\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}NormalStressYZ\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}NormalStressZZ\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{20}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{10}%
\psfrag{x09}[t][t]{20}%
\psfrag{x10}[t][t]{0}%
\psfrag{x11}[t][t]{10}%
\psfrag{x12}[t][t]{20}%
\psfrag{x13}[t][t]{0}%
\psfrag{x14}[t][t]{10}%
\psfrag{x15}[t][t]{20}%
\psfrag{x16}[t][t]{0}%
\psfrag{x17}[t][t]{10}%
\psfrag{x18}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{-0.1}%
\psfrag{v06}[r][r]{-0.05}%
\psfrag{v07}[r][r]{0}%
\psfrag{v08}[r][r]{0.05}%
\psfrag{v09}[r][r]{0}%
\psfrag{v10}[r][r]{5}%
\psfrag{v11}[r][r]{10}%
\psfrag{v12}[r][r]{15}%
\psfrag{v13}[r][r]{-6}%
\psfrag{v14}[r][r]{-4}%
\psfrag{v15}[r][r]{-2}%
\psfrag{v16}[r][r]{0}%
\psfrag{v17}[r][r]{0}%
\psfrag{v18}[r][r]{0.5}%
\psfrag{v19}[r][r]{1}%
\psfrag{v20}[r][r]{1.5}%
\psfrag{v21}[r][r]{0}%
\psfrag{v22}[r][r]{10}%
\psfrag{v23}[r][r]{20}%
%
% Figure:
\resizebox{16cm}{!}{\includegraphics{fstatVsTav_NormalStress.matlab.eps}}%
\end{psfrags}%
%
% End fstatVsTav_NormalStress.matlab.tex


==> Figures/fstatVsTav_TangentialStress.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}TangentialStressXX\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}TangentialStressXY\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}TangentialStressXZ\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}TangentialStressYX\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}TangentialStressYY\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}TangentialStressYZ\end{tabular}}%
\psfrag{s07}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}TangentialStressZX\end{tabular}}%
\psfrag{s08}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}TangentialStressZY\end{tabular}}%
\psfrag{s09}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}TangentialStressZZ\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{20}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{10}%
\psfrag{x09}[t][t]{20}%
\psfrag{x10}[t][t]{0}%
\psfrag{x11}[t][t]{10}%
\psfrag{x12}[t][t]{20}%
\psfrag{x13}[t][t]{0}%
\psfrag{x14}[t][t]{10}%
\psfrag{x15}[t][t]{20}%
\psfrag{x16}[t][t]{0}%
\psfrag{x17}[t][t]{10}%
\psfrag{x18}[t][t]{20}%
\psfrag{x19}[t][t]{0}%
\psfrag{x20}[t][t]{10}%
\psfrag{x21}[t][t]{20}%
\psfrag{x22}[t][t]{0}%
\psfrag{x23}[t][t]{10}%
\psfrag{x24}[t][t]{20}%
\psfrag{x25}[t][t]{0}%
\psfrag{x26}[t][t]{10}%
\psfrag{x27}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{-0.05}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{0.05}%
\psfrag{v07}[r][r]{-1}%
\psfrag{v08}[r][r]{-0.5}%
\psfrag{v09}[r][r]{0}%
\psfrag{v10}[r][r]{-0.05}%
\psfrag{v11}[r][r]{0}%
\psfrag{v12}[r][r]{0.05}%
\psfrag{v13}[r][r]{-0.4}%
\psfrag{v14}[r][r]{-0.2}%
\psfrag{v15}[r][r]{0}%
\psfrag{v16}[r][r]{-0.05}%
\psfrag{v17}[r][r]{0}%
\psfrag{v18}[r][r]{0.05}%
\psfrag{v19}[r][r]{-1}%
\psfrag{v20}[r][r]{-0.5}%
\psfrag{v21}[r][r]{0}%
\psfrag{v22}[r][r]{-0.05}%
\psfrag{v23}[r][r]{0}%
\psfrag{v24}[r][r]{0.05}%
\psfrag{v25}[r][r]{0}%
\psfrag{v26}[r][r]{0.1}%
\psfrag{v27}[r][r]{0.2}%
%
% Figure:
\resizebox{16cm}{!}{\includegraphics{fstatVsTav_TangentialStress.matlab.eps}}%
\end{psfrags}%
%
% End fstatVsTav_TangentialStress.matlab.tex


==> Figures/hstop.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{18}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{24}%
\psfrag{x05}[t][t]{26}%
\psfrag{x06}[t][t]{28}%
\psfrag{x07}[t][t]{30}%
\psfrag{x08}[t][t]{32}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
\psfrag{v09}[r][r]{40}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{hstop.matlab.eps}}%
\end{psfrags}%
%
% End hstop.matlab.tex


==> Figures/lambdaNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rho$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=3/4$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=5/4$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=3/2$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=7/4$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.4}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.4}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{lambdaNu.matlab.eps}}%
\end{psfrags}%
%
% End lambdaNu.matlab.tex


==> Figures/lambdaVelocityX.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=3/4$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=1$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=5/4$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=3/2$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=7/4$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda/d=2$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{lambdaVelocityX.matlab.eps}}%
\end{psfrags}%
%
% End lambdaVelocityX.matlab.tex


==> Figures/muMacro.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\mu_{macro}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=8$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=1/8$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=1/4$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=1/2$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=1$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=2$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=4$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=8$}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s15}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.4}%
\psfrag{v02}[r][r]{0.45}%
\psfrag{v03}[r][r]{0.5}%
\psfrag{v04}[r][r]{0.55}%
\psfrag{v05}[r][r]{0.6}%
\psfrag{v06}[r][r]{0.65}%
\psfrag{v07}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{muMacro.matlab.eps}}%
\end{psfrags}%
%
% End muMacro.matlab.tex


==> Figures/pvdNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rho$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$V=\pi/6\pm40\%$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$V=\pi/6$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$V=\pi/6\pm40\%$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{pvdNu.matlab.eps}}%
\end{psfrags}%
%
% End pvdNu.matlab.tex


==> Figures/pvdVelocityX.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$V=\pi/6\pm40\%$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$V=\pi/6$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$V=\pi/6\pm40\%$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{22}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{pvdVelocityX.matlab.eps}}%
\end{psfrags}%
%
% End pvdVelocityX.matlab.tex


==> Figures/stdW.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}w=w1}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}w=w0.2}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}w=w0.4}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}w=w0.6}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}w=w0.8}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}w=w1}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{stdW.matlab.eps}}%
\end{psfrags}%
%
% End stdW.matlab.tex


==> Figures/stressRatio.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}/\sigma_{zz}$ and $-t_x/t_z$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=8$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=1/8$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=1/4$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=1/2$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=1$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=2$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=4$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu_c=8$}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s15}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.4}%
\psfrag{v02}[r][r]{0.45}%
\psfrag{v03}[r][r]{0.5}%
\psfrag{v04}[r][r]{0.55}%
\psfrag{v05}[r][r]{0.6}%
\psfrag{v06}[r][r]{0.65}%
\psfrag{v07}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{stressRatio.matlab.eps}}%
\end{psfrags}%
%
% End stressRatio.matlab.tex


==> Figures/thetahCoordinationNumber.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$tr(F)$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{6}%
\psfrag{x05}[t][t]{8}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{12}%
\psfrag{x08}[t][t]{14}%
\psfrag{x09}[t][t]{16}%
\psfrag{x10}[t][t]{18}%
\psfrag{x11}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
\psfrag{v06}[r][r]{2.5}%
\psfrag{v07}[r][r]{3}%
\psfrag{v08}[r][r]{3.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahCoordinationNumber.matlab.eps}}%
\end{psfrags}%
%
% End thetahCoordinationNumber.matlab.tex


==> Figures/thetahFabricAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$|F_{xz}/tr(F)|$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{5}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{15}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{30}%
\psfrag{x07}[t][t]{35}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.08}%
\psfrag{v02}[r][r]{0.09}%
\psfrag{v03}[r][r]{0.1}%
\psfrag{v04}[r][r]{0.11}%
\psfrag{v05}[r][r]{0.12}%
\psfrag{v06}[r][r]{0.13}%
\psfrag{v07}[r][r]{0.14}%
\psfrag{v08}[r][r]{0.15}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahFabricAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End thetahFabricAnisotropy.matlab.tex


==> Figures/thetahFlowPrincipalStressOrientation.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_{\sigma_1}$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_{\sigma_2}$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_{\sigma_3}$\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{5}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{15}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{30}%
\psfrag{x07}[t][t]{35}%
\psfrag{x08}[t][t]{5}%
\psfrag{x09}[t][t]{10}%
\psfrag{x10}[t][t]{15}%
\psfrag{x11}[t][t]{20}%
\psfrag{x12}[t][t]{25}%
\psfrag{x13}[t][t]{30}%
\psfrag{x14}[t][t]{35}%
\psfrag{x15}[t][t]{5}%
\psfrag{x16}[t][t]{10}%
\psfrag{x17}[t][t]{15}%
\psfrag{x18}[t][t]{20}%
\psfrag{x19}[t][t]{25}%
\psfrag{x20}[t][t]{30}%
\psfrag{x21}[t][t]{35}%
%
% yticklabels:
\psfrag{v01}[r][r]{45}%
\psfrag{v02}[r][r]{50}%
\psfrag{v03}[r][r]{55}%
\psfrag{v04}[r][r]{-50}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{50}%
\psfrag{v07}[r][r]{-45}%
\psfrag{v08}[r][r]{-40}%
\psfrag{v09}[r][r]{-35}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahFlowPrincipalStressOrientation.matlab.eps}}%
\end{psfrags}%
%
% End thetahFlowPrincipalStressOrientation.matlab.tex


==> Figures/thetahGamma.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=18^\circ$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=22^\circ$\end{tabular}}%
\psfrag{s05}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$\end{tabular}}%
\psfrag{s07}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=26^\circ$\end{tabular}}%
\psfrag{s08}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s09}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$\end{tabular}}%
\psfrag{s10}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=30^\circ$\end{tabular}}%
\psfrag{s11}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s12}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$\end{tabular}}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40d$}%
\psfrag{s15}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=5d$}%
\psfrag{s16}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10d$}%
\psfrag{s17}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20d$}%
\psfrag{s18}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40d$}%
\psfrag{s20}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s21}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{5}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{15}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{30}%
\psfrag{x07}[t][t]{5}%
\psfrag{x08}[t][t]{10}%
\psfrag{x09}[t][t]{15}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{25}%
\psfrag{x12}[t][t]{30}%
\psfrag{x13}[t][t]{5}%
\psfrag{x14}[t][t]{10}%
\psfrag{x15}[t][t]{15}%
\psfrag{x16}[t][t]{20}%
\psfrag{x17}[t][t]{25}%
\psfrag{x18}[t][t]{30}%
\psfrag{x19}[t][t]{5}%
\psfrag{x20}[t][t]{10}%
\psfrag{x21}[t][t]{15}%
\psfrag{x22}[t][t]{20}%
\psfrag{x23}[t][t]{25}%
\psfrag{x24}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{1}%
\psfrag{v02}[r][r]{1.5}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{0.2}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.6}%
\psfrag{v07}[r][r]{0.8}%
\psfrag{v08}[r][r]{1}%
\psfrag{v09}[r][r]{0.05}%
\psfrag{v10}[r][r]{0.1}%
\psfrag{v11}[r][r]{0.15}%
\psfrag{v12}[r][r]{0.2}%
\psfrag{v13}[r][r]{0.25}%
\psfrag{v14}[r][r]{0.3}%
\psfrag{v15}[r][r]{0.005}%
\psfrag{v16}[r][r]{0.01}%
\psfrag{v17}[r][r]{0.015}%
%
% Figure:
\resizebox{16cm}{!}{\includegraphics{thetahGamma.matlab.eps}}%
\end{psfrags}%
%
% End thetahGamma.matlab.tex


==> Figures/thetahMu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\mu_{Macro}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$tan(\theta)$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=5d$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10d$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20d$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40d$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$tan(\theta)$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahMu.matlab.eps}}%
\end{psfrags}%
%
% End thetahMu.matlab.tex


==> Figures/thetahMuMacro.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\mu_{Macro}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$tan(\theta)$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=5d$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10d$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20d$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40d$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$tan(\theta)$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{1.5}%
\psfrag{v04}[r][r]{2}%
\psfrag{v05}[r][r]{2.5}%
\psfrag{v06}[r][r]{3}%
\psfrag{v07}[r][r]{3.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahMuMacro.matlab.eps}}%
\end{psfrags}%
%
% End thetahMuMacro.matlab.tex


==> Figures/thetahNu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{2}%
\psfrag{x02}[t][t]{4}%
\psfrag{x03}[t][t]{6}%
\psfrag{x04}[t][t]{8}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{12}%
\psfrag{x07}[t][t]{14}%
\psfrag{x08}[t][t]{16}%
\psfrag{x09}[t][t]{18}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahNu.matlab.eps}}%
\end{psfrags}%
%
% End thetahNu.matlab.tex


==> Figures/thetahPressureAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{xx}/p$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{yy}/p$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{zz}/p$\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{5}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{15}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{30}%
\psfrag{x07}[t][t]{35}%
\psfrag{x08}[t][t]{5}%
\psfrag{x09}[t][t]{10}%
\psfrag{x10}[t][t]{15}%
\psfrag{x11}[t][t]{20}%
\psfrag{x12}[t][t]{25}%
\psfrag{x13}[t][t]{30}%
\psfrag{x14}[t][t]{35}%
\psfrag{x15}[t][t]{5}%
\psfrag{x16}[t][t]{10}%
\psfrag{x17}[t][t]{15}%
\psfrag{x18}[t][t]{20}%
\psfrag{x19}[t][t]{25}%
\psfrag{x20}[t][t]{30}%
\psfrag{x21}[t][t]{35}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.9}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{1.1}%
\psfrag{v04}[r][r]{0.7}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{0.9}%
\psfrag{v07}[r][r]{1}%
\psfrag{v08}[r][r]{1.05}%
\psfrag{v09}[r][r]{1.1}%
\psfrag{v10}[r][r]{1.15}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahPressureAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End thetahPressureAnisotropy.matlab.tex


==> Figures/thetahPressureUniformity.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{ii}/p$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{zz}/p$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{xx}/p$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{yy}/p$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{zz}/p$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.1}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.3}%
\psfrag{x04}[t][t]{0.4}%
\psfrag{x05}[t][t]{0.5}%
\psfrag{x06}[t][t]{0.6}%
\psfrag{x07}[t][t]{0.7}%
\psfrag{x08}[t][t]{0.8}%
\psfrag{x09}[t][t]{0.9}%
\psfrag{x10}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.75}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{1.25}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahPressureUniformity.matlab.eps}}%
\end{psfrags}%
%
% End thetahPressureUniformity.matlab.tex


==> Figures/thetahPrincipalPressureAnisotropy.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_1/p$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_2/p$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_3/p$\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{5}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{15}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{30}%
\psfrag{x07}[t][t]{35}%
\psfrag{x08}[t][t]{5}%
\psfrag{x09}[t][t]{10}%
\psfrag{x10}[t][t]{15}%
\psfrag{x11}[t][t]{20}%
\psfrag{x12}[t][t]{25}%
\psfrag{x13}[t][t]{30}%
\psfrag{x14}[t][t]{35}%
\psfrag{x15}[t][t]{5}%
\psfrag{x16}[t][t]{10}%
\psfrag{x17}[t][t]{15}%
\psfrag{x18}[t][t]{20}%
\psfrag{x19}[t][t]{25}%
\psfrag{x20}[t][t]{30}%
\psfrag{x21}[t][t]{35}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{0.55}%
\psfrag{v03}[r][r]{0.6}%
\psfrag{v04}[r][r]{0.7}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{0.9}%
\psfrag{v07}[r][r]{1}%
\psfrag{v08}[r][r]{1.5}%
\psfrag{v09}[r][r]{1.6}%
\psfrag{v10}[r][r]{1.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahPrincipalPressureAnisotropy.matlab.eps}}%
\end{psfrags}%
%
% End thetahPrincipalPressureAnisotropy.matlab.tex


==> Figures/thetahPrincipalStressOrientation.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_{\sigma_1}$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_{\sigma_2}$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_{\sigma_3}$\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.2}%
\psfrag{x02}[t][t]{0.4}%
\psfrag{x03}[t][t]{0.6}%
\psfrag{x04}[t][t]{0.8}%
\psfrag{x05}[t][t]{1}%
\psfrag{x06}[t][t]{0.2}%
\psfrag{x07}[t][t]{0.4}%
\psfrag{x08}[t][t]{0.6}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{1}%
\psfrag{x11}[t][t]{0.2}%
\psfrag{x12}[t][t]{0.4}%
\psfrag{x13}[t][t]{0.6}%
\psfrag{x14}[t][t]{0.8}%
\psfrag{x15}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{-50}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{50}%
\psfrag{v04}[r][r]{-50}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{50}%
\psfrag{v07}[r][r]{-50}%
\psfrag{v08}[r][r]{0}%
\psfrag{v09}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahPrincipalStressOrientation.matlab.eps}}%
\end{psfrags}%
%
% End thetahPrincipalStressOrientation.matlab.tex


==> Figures/thetahPrincipalStressOrientation2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_{\max}$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\phi_{\min}$\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
\psfrag{x08}[t][t]{35}%
\psfrag{x09}[t][t]{40}%
\psfrag{x10}[t][t]{0}%
\psfrag{x11}[t][t]{5}%
\psfrag{x12}[t][t]{10}%
\psfrag{x13}[t][t]{15}%
\psfrag{x14}[t][t]{20}%
\psfrag{x15}[t][t]{25}%
\psfrag{x16}[t][t]{30}%
\psfrag{x17}[t][t]{35}%
\psfrag{x18}[t][t]{40}%
%
% yticklabels:
\psfrag{v01}[r][r]{44}%
\psfrag{v02}[r][r]{46}%
\psfrag{v03}[r][r]{48}%
\psfrag{v04}[r][r]{50}%
\psfrag{v05}[r][r]{52}%
\psfrag{v06}[r][r]{-46}%
\psfrag{v07}[r][r]{-44}%
\psfrag{v08}[r][r]{-42}%
\psfrag{v09}[r][r]{-40}%
\psfrag{v10}[r][r]{-38}%
\psfrag{v11}[r][r]{-36}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahPrincipalStressOrientation2.matlab.eps}}%
\end{psfrags}%
%
% End thetahPrincipalStressOrientation2.matlab.tex


==> Figures/thetahSDoverGamma.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=18^\circ$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma^2$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=22^\circ$\end{tabular}}%
\psfrag{s05}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma^2$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}$\end{tabular}}%
\psfrag{s07}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=26^\circ$\end{tabular}}%
\psfrag{s08}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma^2$\end{tabular}}%
\psfrag{s09}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}$\end{tabular}}%
\psfrag{s10}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=30^\circ$\end{tabular}}%
\psfrag{s11}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma^2$\end{tabular}}%
\psfrag{s12}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}$\end{tabular}}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40d$}%
\psfrag{s15}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=5d$}%
\psfrag{s16}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10d$}%
\psfrag{s17}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20d$}%
\psfrag{s18}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40d$}%
\psfrag{s20}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s21}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{1}%
\psfrag{x02}[t][t]{2}%
\psfrag{x03}[t][t]{3}%
\psfrag{x04}[t][t]{4}%
\psfrag{x05}[t][t]{5}%
\psfrag{x06}[t][t]{6}%
\psfrag{x07}[t][t]{0.2}%
\psfrag{x08}[t][t]{0.4}%
\psfrag{x09}[t][t]{0.6}%
\psfrag{x10}[t][t]{0.8}%
\psfrag{x11}[t][t]{1}%
\psfrag{x12}[t][t]{0.02}%
\psfrag{x13}[t][t]{0.04}%
\psfrag{x14}[t][t]{0.06}%
\psfrag{x15}[t][t]{0.08}%
\psfrag{x16}[t][t]{0.1}%
\psfrag{x17}[t][t]{1}%
\psfrag{x18}[t][t]{2}%
\psfrag{x19}[t][t]{3}%
\psfrag{x20}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{10}%
\psfrag{v08}[r][r]{15}%
\psfrag{v09}[r][r]{0}%
\psfrag{v10}[r][r]{5}%
\psfrag{v11}[r][r]{10}%
\psfrag{v12}[r][r]{15}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{5}%
\psfrag{v15}[r][r]{10}%
\psfrag{v16}[r][r]{15}%
%
% Figure:
\resizebox{16cm}{!}{\includegraphics{thetahSDoverGamma.matlab.eps}}%
\end{psfrags}%
%
% End thetahSDoverGamma.matlab.tex


==> Figures/thetahStressXZoverPressure.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=18^\circ$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$p$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=22^\circ$\end{tabular}}%
\psfrag{s05}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$p$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}$\end{tabular}}%
\psfrag{s07}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=26^\circ$\end{tabular}}%
\psfrag{s08}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$p$\end{tabular}}%
\psfrag{s09}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}$\end{tabular}}%
\psfrag{s10}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta=30^\circ$\end{tabular}}%
\psfrag{s11}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$p$\end{tabular}}%
\psfrag{s12}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$-\sigma_{xz}$\end{tabular}}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40d$}%
\psfrag{s15}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=5d$}%
\psfrag{s16}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10d$}%
\psfrag{s17}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20d$}%
\psfrag{s18}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40d$}%
\psfrag{s20}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s21}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{5}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{15}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{30}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{10}%
\psfrag{x09}[t][t]{20}%
\psfrag{x10}[t][t]{30}%
\psfrag{x11}[t][t]{10}%
\psfrag{x12}[t][t]{20}%
\psfrag{x13}[t][t]{30}%
\psfrag{x14}[t][t]{10}%
\psfrag{x15}[t][t]{20}%
\psfrag{x16}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{5}%
\psfrag{v02}[r][r]{10}%
\psfrag{v03}[r][r]{15}%
\psfrag{v04}[r][r]{5}%
\psfrag{v05}[r][r]{10}%
\psfrag{v06}[r][r]{15}%
\psfrag{v07}[r][r]{0}%
\psfrag{v08}[r][r]{5}%
\psfrag{v09}[r][r]{10}%
\psfrag{v10}[r][r]{2}%
\psfrag{v11}[r][r]{4}%
\psfrag{v12}[r][r]{6}%
\psfrag{v13}[r][r]{8}%
\psfrag{v14}[r][r]{10}%
\psfrag{v15}[r][r]{12}%
%
% Figure:
\resizebox{16cm}{!}{\includegraphics{thetahStressXZoverPressure.matlab.eps}}%
\end{psfrags}%
%
% End thetahStressXZoverPressure.matlab.tex


==> Figures/thetahStressZZ.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{zz}/(\int\!\!\rho g\, dz)$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40d$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=5d$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10d$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20d$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40d$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahStressZZ.matlab.eps}}%
\end{psfrags}%
%
% End thetahStressZZ.matlab.tex


==> Figures/thetahTotalSD.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$s_D$ and $s_D^\star$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=18^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{5}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{15}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{30}%
\psfrag{x07}[t][t]{35}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.35}%
\psfrag{v02}[r][r]{0.4}%
\psfrag{v03}[r][r]{0.45}%
\psfrag{v04}[r][r]{0.5}%
\psfrag{v05}[r][r]{0.55}%
\psfrag{v06}[r][r]{0.6}%
\psfrag{v07}[r][r]{0.65}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahTotalSD.matlab.eps}}%
\end{psfrags}%
%
% End thetahTotalSD.matlab.tex


==> Figures/thetahVelocityX.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$u/\bar{u}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.2}%
\psfrag{v02}[r][r]{0.4}%
\psfrag{v03}[r][r]{0.6}%
\psfrag{v04}[r][r]{0.8}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{1.2}%
\psfrag{v07}[r][r]{1.4}%
\psfrag{v08}[r][r]{1.6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahVelocityX.matlab.eps}}%
\end{psfrags}%
%
% End thetahVelocityX.matlab.tex


==> Figures/thetahZ.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$tr(F)$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{5}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{15}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{30}%
\psfrag{x07}[t][t]{35}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
\psfrag{v06}[r][r]{2.5}%
\psfrag{v07}[r][r]{3}%
\psfrag{v08}[r][r]{3.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{thetahZ.matlab.eps}}%
\end{psfrags}%
%
% End thetahZ.matlab.tex


==> FiguresMatlab/accelerating_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$E_{kin}(t)/E_{kin}(2000)$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{1955}%
\psfrag{x02}[t][t]{1960}%
\psfrag{x03}[t][t]{1965}%
\psfrag{x04}[t][t]{1970}%
\psfrag{x05}[t][t]{1975}%
\psfrag{x06}[t][t]{1980}%
\psfrag{x07}[t][t]{1985}%
\psfrag{x08}[t][t]{1990}%
\psfrag{x09}[t][t]{1995}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.92}%
\psfrag{v02}[r][r]{0.94}%
\psfrag{v03}[r][r]{0.96}%
\psfrag{v04}[r][r]{0.98}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{1.02}%
\psfrag{v07}[r][r]{1.04}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{accelerating_5.matlab.eps}}%
\end{psfrags}%
%
% End accelerating_5.matlab.tex


==> FiguresMatlab/arresting.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$E_{kin}/\langle{E}_{ela}\rangle$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=20^\circ$}%
\psfrag{s06}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=60^\circ$}%
\psfrag{s07}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=50^\circ$}%
\psfrag{s08}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=40^\circ$}%
\psfrag{s09}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s10}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=29^\circ$}%
\psfrag{s11}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s12}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s13}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s14}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s15}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s16}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s17}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s18}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=21.5^\circ$}%
\psfrag{s19}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=21^\circ$}%
\psfrag{s20}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=20.5^\circ$}%
\psfrag{s21}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=20^\circ$}%
\psfrag{s23}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s24}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{8}{12}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{500}%
\psfrag{x03}[t][t]{1000}%
\psfrag{x04}[t][t]{1500}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{0}$}%
\psfrag{v02}[r][r]{$10^{1}$}%
\psfrag{v03}[r][r]{$10^{2}$}%
\psfrag{v04}[r][r]{$10^{3}$}%
\psfrag{v05}[r][r]{$10^{4}$}%
\psfrag{v06}[r][r]{$10^{5}$}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{arresting.matlab.eps}}%
\end{psfrags}%
%
% End arresting.matlab.tex


==> FiguresMatlab/arresting_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$t$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$E_{kin}/\overline{E}_{ela}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=60^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=20^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s15}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=40^\circ$}%
\psfrag{s16}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=50^\circ$}%
\psfrag{s17}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=60^\circ$}%
\psfrag{s19}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s20}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{500}%
\psfrag{x03}[t][t]{1000}%
\psfrag{x04}[t][t]{1500}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{0}$}%
\psfrag{v02}[r][r]{$10^{1}$}%
\psfrag{v03}[r][r]{$10^{2}$}%
\psfrag{v04}[r][r]{$10^{3}$}%
\psfrag{v05}[r][r]{$10^{4}$}%
\psfrag{v06}[r][r]{$10^{5}$}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{arresting_5.matlab.eps}}%
\end{psfrags}%
%
% End arresting_5.matlab.tex


==> FiguresMatlab/cg.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\rho$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-2}%
\psfrag{x02}[t][t]{-1.5}%
\psfrag{x03}[t][t]{-1}%
\psfrag{x04}[t][t]{-0.5}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{1}%
\psfrag{x08}[t][t]{1.5}%
\psfrag{x09}[t][t]{2}%
\psfrag{x10}[t][t]{2.5}%
\psfrag{x11}[t][t]{3}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{cg.matlab.eps}}%
\end{psfrags}%
%
% End cg.matlab.tex


==> FiguresMatlab/cg2_new.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\partial_x \sigma$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\rho$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\partial_x \sigma$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-2}%
\psfrag{x02}[t][t]{-1}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{1}%
\psfrag{x05}[t][t]{2}%
%
% yticklabels:
\psfrag{v01}[r][r]{-2}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{cg2_new.matlab.eps}}%
\end{psfrags}%
%
% End cg2_new.matlab.tex


==> FiguresMatlab/cg_new.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\partial_x \sigma$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\rho$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\partial_x \sigma$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-2}%
\psfrag{x02}[t][t]{-1}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{1}%
\psfrag{x05}[t][t]{2}%
%
% yticklabels:
\psfrag{v01}[r][r]{-2}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{cg_new.matlab.eps}}%
\end{psfrags}%
%
% End cg_new.matlab.tex


==> FiguresMatlab/codestatus_flow_1_2_3_4_5_6.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=0$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1/2$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=2/3$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=5/6$\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=2$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{40}%
\psfrag{x03}[t][t]{60}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{40}%
\psfrag{x06}[t][t]{60}%
\psfrag{x07}[t][t]{20}%
\psfrag{x08}[t][t]{40}%
\psfrag{x09}[t][t]{60}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{40}%
\psfrag{x12}[t][t]{60}%
\psfrag{x13}[t][t]{20}%
\psfrag{x14}[t][t]{40}%
\psfrag{x15}[t][t]{60}%
\psfrag{x16}[t][t]{20}%
\psfrag{x17}[t][t]{40}%
\psfrag{x18}[t][t]{60}%
%
% yticklabels:
\psfrag{v01}[r][r]{10}%
\psfrag{v02}[r][r]{20}%
\psfrag{v03}[r][r]{30}%
\psfrag{v04}[r][r]{40}%
\psfrag{v05}[r][r]{10}%
\psfrag{v06}[r][r]{20}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{40}%
\psfrag{v09}[r][r]{10}%
\psfrag{v10}[r][r]{20}%
\psfrag{v11}[r][r]{30}%
\psfrag{v12}[r][r]{40}%
\psfrag{v13}[r][r]{10}%
\psfrag{v14}[r][r]{20}%
\psfrag{v15}[r][r]{30}%
\psfrag{v16}[r][r]{40}%
\psfrag{v17}[r][r]{10}%
\psfrag{v18}[r][r]{20}%
\psfrag{v19}[r][r]{30}%
\psfrag{v20}[r][r]{40}%
\psfrag{v21}[r][r]{10}%
\psfrag{v22}[r][r]{20}%
\psfrag{v23}[r][r]{30}%
\psfrag{v24}[r][r]{40}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{codestatus_flow_1_2_3_4_5_6.matlab.eps}}%
\end{psfrags}%
%
% End codestatus_flow_1_2_3_4_5_6.matlab.tex


==> FiguresMatlab/codestatus_flow_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{25}%
\psfrag{x03}[t][t]{30}%
\psfrag{x04}[t][t]{35}%
\psfrag{x05}[t][t]{40}%
\psfrag{x06}[t][t]{45}%
\psfrag{x07}[t][t]{50}%
\psfrag{x08}[t][t]{55}%
\psfrag{x09}[t][t]{60}%
%
% yticklabels:
\psfrag{v01}[r][r]{10}%
\psfrag{v02}[r][r]{15}%
\psfrag{v03}[r][r]{20}%
\psfrag{v04}[r][r]{25}%
\psfrag{v05}[r][r]{30}%
\psfrag{v06}[r][r]{35}%
\psfrag{v07}[r][r]{40}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{codestatus_flow_5.matlab.eps}}%
\end{psfrags}%
%
% End codestatus_flow_5.matlab.tex


==> FiguresMatlab/codestatus_hstop_1_2_3_4_5_6.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=0$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1/2$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=2/3$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=5/6$\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=2$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{15}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{25}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{15}%
\psfrag{x08}[t][t]{20}%
\psfrag{x09}[t][t]{25}%
\psfrag{x10}[t][t]{15}%
\psfrag{x11}[t][t]{20}%
\psfrag{x12}[t][t]{25}%
\psfrag{x13}[t][t]{18}%
\psfrag{x14}[t][t]{20}%
\psfrag{x15}[t][t]{22}%
\psfrag{x16}[t][t]{10}%
\psfrag{x17}[t][t]{15}%
\psfrag{x18}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{10}%
\psfrag{v03}[r][r]{20}%
\psfrag{v04}[r][r]{30}%
\psfrag{v05}[r][r]{40}%
\psfrag{v06}[r][r]{0}%
\psfrag{v07}[r][r]{20}%
\psfrag{v08}[r][r]{40}%
\psfrag{v09}[r][r]{60}%
\psfrag{v10}[r][r]{0}%
\psfrag{v11}[r][r]{10}%
\psfrag{v12}[r][r]{20}%
\psfrag{v13}[r][r]{30}%
\psfrag{v14}[r][r]{40}%
\psfrag{v15}[r][r]{50}%
\psfrag{v16}[r][r]{0}%
\psfrag{v17}[r][r]{20}%
\psfrag{v18}[r][r]{40}%
\psfrag{v19}[r][r]{60}%
\psfrag{v20}[r][r]{0}%
\psfrag{v21}[r][r]{20}%
\psfrag{v22}[r][r]{40}%
\psfrag{v23}[r][r]{60}%
\psfrag{v24}[r][r]{0}%
\psfrag{v25}[r][r]{20}%
\psfrag{v26}[r][r]{40}%
\psfrag{v27}[r][r]{60}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{codestatus_hstop_1_2_3_4_5_6.matlab.eps}}%
\end{psfrags}%
%
% End codestatus_hstop_1_2_3_4_5_6.matlab.tex


==> FiguresMatlab/codestatus_hstop_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}L1\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{18}%
\psfrag{x02}[t][t]{19}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{21}%
\psfrag{x05}[t][t]{22}%
\psfrag{x06}[t][t]{23}%
\psfrag{x07}[t][t]{24}%
\psfrag{x08}[t][t]{25}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{10}%
\psfrag{v03}[r][r]{20}%
\psfrag{v04}[r][r]{30}%
\psfrag{v05}[r][r]{40}%
\psfrag{v06}[r][r]{50}%
\psfrag{v07}[r][r]{60}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{codestatus_hstop_5.matlab.eps}}%
\end{psfrags}%
%
% End codestatus_hstop_5.matlab.tex


==> FiguresMatlab/coeffhstop.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta_2$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta_1$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta_2$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0.5}%
\psfrag{x02}[t][t]{1}%
\psfrag{x03}[t][t]{1.5}%
\psfrag{x04}[t][t]{2}%
%
% yticklabels:
\psfrag{v01}[r][r]{18}%
\psfrag{v02}[r][r]{20}%
\psfrag{v03}[r][r]{22}%
\psfrag{v04}[r][r]{24}%
\psfrag{v05}[r][r]{26}%
\psfrag{v06}[r][r]{28}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{32}%
\psfrag{v09}[r][r]{34}%
\psfrag{v10}[r][r]{36}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{coeffhstop.matlab.eps}}%
\end{psfrags}%
%
% End coeffhstop.matlab.tex


==> FiguresMatlab/depthprofile_NormalStresses_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=24^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=26^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=28^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=30^\circ$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{0.6}%
\psfrag{v03}[r][r]{0.7}%
\psfrag{v04}[r][r]{0.8}%
\psfrag{v05}[r][r]{0.9}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.1}%
\psfrag{v08}[r][r]{1.2}%
\psfrag{v09}[r][r]{1.3}%
\psfrag{v10}[r][r]{1.4}%
\psfrag{v11}[r][r]{1.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_NormalStresses_5.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_NormalStresses_5.matlab.tex


==> FiguresMatlab/depthprofile_NormalStresses_5H30A26.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}surface}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{xx}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{yy}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{zz}$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}base}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}surface}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
\psfrag{x08}[t][t]{35}%
\psfrag{x09}[t][t]{40}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_NormalStresses_5H30A26.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_NormalStresses_5H30A26.matlab.tex


==> FiguresMatlab/depthprofile_NormalStresses_5H30A30.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z-b$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\leftarrow\sigma_{xx}$\end{tabular}}%
\psfrag{s06}[r][r]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{r}$\sigma_{zz}\rightarrow$\end{tabular}}%
\psfrag{s07}[r][r]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{r}$\sigma_{yy}\rightarrow$\end{tabular}}%
\psfrag{s08}[r][r]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{r}$-\sigma_{xz}\rightarrow$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
\psfrag{x08}[t][t]{35}%
%
% yticklabels:
\psfrag{v01}[r][r]{5}%
\psfrag{v02}[r][r]{10}%
\psfrag{v03}[r][r]{15}%
\psfrag{v04}[r][r]{20}%
\psfrag{v05}[r][r]{25}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_NormalStresses_5H30A30.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_NormalStresses_5H30A30.matlab.tex


==> FiguresMatlab/depthprofile_NormalStresses_5_H_20.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\sigma_{xx}/\sigma_{zz}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s08}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s09}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{8}{12}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.8}%
\psfrag{v02}[r][r]{0.9}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.1}%
\psfrag{v05}[r][r]{1.2}%
\psfrag{v06}[r][r]{1.3}%
\psfrag{v07}[r][r]{1.4}%
\psfrag{v08}[r][r]{1.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_NormalStresses_5_H_20.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_NormalStresses_5_H_20.matlab.tex


==> FiguresMatlab/depthprofile_Nu_2_H_30.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.4}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.4}%
\psfrag{v09}[r][r]{1.6}%
\psfrag{v10}[r][r]{1.8}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_Nu_2_H_30.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_Nu_2_H_30.matlab.tex


==> FiguresMatlab/depthprofile_Nu_3_H_30.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_Nu_3_H_30.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_Nu_3_H_30.matlab.tex


==> FiguresMatlab/depthprofile_Nu_5_H_30.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_Nu_5_H_30.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_Nu_5_H_30.matlab.tex


==> FiguresMatlab/depthprofile_VelocityX_2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10,\theta=28^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10,\theta=20^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10,\theta=21^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10,\theta=22^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10,\theta=23^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10,\theta=24^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10,\theta=26^\circ$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10,\theta=28^\circ$}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s15}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s16}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s17}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s20}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=28^\circ$}%
\psfrag{s21}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=20^\circ$}%
\psfrag{s22}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=21^\circ$}%
\psfrag{s23}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=22^\circ$}%
\psfrag{s24}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=23^\circ$}%
\psfrag{s25}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=24^\circ$}%
\psfrag{s26}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=26^\circ$}%
\psfrag{s27}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=28^\circ$}%
\psfrag{s29}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s30}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s31}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s32}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s35}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=30,\theta=28^\circ$}%
\psfrag{s36}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=30,\theta=20^\circ$}%
\psfrag{s37}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=30,\theta=22^\circ$}%
\psfrag{s38}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=30,\theta=24^\circ$}%
\psfrag{s39}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=30,\theta=26^\circ$}%
\psfrag{s40}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=30,\theta=28^\circ$}%
\psfrag{s42}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s43}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s44}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s45}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s48}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40,\theta=28^\circ$}%
\psfrag{s49}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40,\theta=20^\circ$}%
\psfrag{s50}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40,\theta=22^\circ$}%
\psfrag{s51}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40,\theta=24^\circ$}%
\psfrag{s52}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40,\theta=26^\circ$}%
\psfrag{s53}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40,\theta=28^\circ$}%
\psfrag{s55}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s56}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{0.2}%
\psfrag{x09}[t][t]{0.4}%
\psfrag{x10}[t][t]{0.6}%
\psfrag{x11}[t][t]{0.8}%
\psfrag{x12}[t][t]{1}%
\psfrag{x13}[t][t]{0}%
\psfrag{x14}[t][t]{0.2}%
\psfrag{x15}[t][t]{0.4}%
\psfrag{x16}[t][t]{0.6}%
\psfrag{x17}[t][t]{0.8}%
\psfrag{x18}[t][t]{1}%
\psfrag{x19}[t][t]{0}%
\psfrag{x20}[t][t]{0.2}%
\psfrag{x21}[t][t]{0.4}%
\psfrag{x22}[t][t]{0.6}%
\psfrag{x23}[t][t]{0.8}%
\psfrag{x24}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{1}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{2}%
\psfrag{v08}[r][r]{0}%
\psfrag{v09}[r][r]{1}%
\psfrag{v10}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_VelocityX_2.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_VelocityX_2.matlab.tex


==> FiguresMatlab/depthprofile_VelocityX_2_H_30.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=20^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.4}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.4}%
\psfrag{v09}[r][r]{1.6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_VelocityX_2_H_30.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_VelocityX_2_H_30.matlab.tex


==> FiguresMatlab/depthprofile_VelocityX_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=24^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=26^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=28^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=30^\circ$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{0.6}%
\psfrag{v03}[r][r]{0.7}%
\psfrag{v04}[r][r]{0.8}%
\psfrag{v05}[r][r]{0.9}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.1}%
\psfrag{v08}[r][r]{1.2}%
\psfrag{v09}[r][r]{1.3}%
\psfrag{v10}[r][r]{1.4}%
\psfrag{v11}[r][r]{1.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_VelocityX_5.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_VelocityX_5.matlab.tex


==> FiguresMatlab/depthprofile_VelocityX_5_H_10.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Linear}%
\psfrag{s06}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s07}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s08}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s09}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s10}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s11}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Linear}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{8}{12}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
\psfrag{v06}[r][r]{2.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_VelocityX_5_H_10.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_VelocityX_5_H_10.matlab.tex


==> FiguresMatlab/depthprofile_VelocityX_5_H_20.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold}%
\psfrag{s16}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s17}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_VelocityX_5_H_20.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_VelocityX_5_H_20.matlab.tex


==> FiguresMatlab/depthprofile_VelocityX_5_H_30.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=20^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.1}%
\psfrag{x03}[t][t]{0.2}%
\psfrag{x04}[t][t]{0.3}%
\psfrag{x05}[t][t]{0.4}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{0.6}%
\psfrag{x08}[t][t]{0.7}%
\psfrag{x09}[t][t]{0.8}%
\psfrag{x10}[t][t]{0.9}%
\psfrag{x11}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_VelocityX_5_H_30.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_VelocityX_5_H_30.matlab.tex


==> FiguresMatlab/depthprofile_VelocityX_W05_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v/\overline{v}$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=30^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=20^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=22^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=24^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=26^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=28^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20,\theta=30^\circ$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.4}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.4}%
\psfrag{v09}[r][r]{1.6}%
\psfrag{v10}[r][r]{1.8}%
\psfrag{v11}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{depthprofile_VelocityX_W05_5.matlab.eps}}%
\end{psfrags}%
%
% End depthprofile_VelocityX_W05_5.matlab.tex


==> FiguresMatlab/figure1.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.2}%
\psfrag{v03}[r][r]{0.4}%
\psfrag{v04}[r][r]{0.6}%
\psfrag{v05}[r][r]{0.8}%
\psfrag{v06}[r][r]{1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{figure1.matlab.eps}}%
\end{psfrags}%
%
% End figure1.matlab.tex


==> FiguresMatlab/flow_rule_H_nonsteady_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}h\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}F\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=60^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=30^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=40^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=50^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=60^\circ$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{100}%
\psfrag{x03}[t][t]{200}%
\psfrag{x04}[t][t]{300}%
\psfrag{x05}[t][t]{400}%
\psfrag{x06}[t][t]{500}%
\psfrag{x07}[t][t]{600}%
\psfrag{x08}[t][t]{700}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{10}%
\psfrag{v03}[r][r]{20}%
\psfrag{v04}[r][r]{30}%
\psfrag{v05}[r][r]{40}%
\psfrag{v06}[r][r]{50}%
\psfrag{v07}[r][r]{60}%
\psfrag{v08}[r][r]{70}%
\psfrag{v09}[r][r]{80}%
\psfrag{v10}[r][r]{90}%
\psfrag{v11}[r][r]{100}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{flow_rule_H_nonsteady_5.matlab.eps}}%
\end{psfrags}%
%
% End flow_rule_H_nonsteady_5.matlab.tex


==> FiguresMatlab/flow_rule_h_1_2_3_4_5_6.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}h\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}F\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=0$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}h\end{tabular}}%
\psfrag{s11}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}F\end{tabular}}%
\psfrag{s13}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1/2$\end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s15}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s18}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}h\end{tabular}}%
\psfrag{s19}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}F\end{tabular}}%
\psfrag{s21}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=2/3$\end{tabular}}%
\psfrag{s22}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s23}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s26}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}h\end{tabular}}%
\psfrag{s27}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}F\end{tabular}}%
\psfrag{s29}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=5/6$\end{tabular}}%
\psfrag{s30}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s31}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s34}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}h\end{tabular}}%
\psfrag{s35}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}F\end{tabular}}%
\psfrag{s37}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1$\end{tabular}}%
\psfrag{s38}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s39}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s42}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}h\end{tabular}}%
\psfrag{s43}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}F\end{tabular}}%
\psfrag{s45}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=2$\end{tabular}}%
\psfrag{s46}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s47}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{0}%
\psfrag{x07}[t][t]{0.5}%
\psfrag{x08}[t][t]{1}%
\psfrag{x09}[t][t]{0}%
\psfrag{x10}[t][t]{20}%
\psfrag{x11}[t][t]{0}%
\psfrag{x12}[t][t]{0.5}%
\psfrag{x13}[t][t]{1}%
\psfrag{x14}[t][t]{0}%
\psfrag{x15}[t][t]{20}%
\psfrag{x16}[t][t]{0}%
\psfrag{x17}[t][t]{0.5}%
\psfrag{x18}[t][t]{1}%
\psfrag{x19}[t][t]{0}%
\psfrag{x20}[t][t]{10}%
\psfrag{x21}[t][t]{20}%
\psfrag{x22}[t][t]{0}%
\psfrag{x23}[t][t]{0.5}%
\psfrag{x24}[t][t]{1}%
\psfrag{x25}[t][t]{0}%
\psfrag{x26}[t][t]{10}%
\psfrag{x27}[t][t]{20}%
\psfrag{x28}[t][t]{0}%
\psfrag{x29}[t][t]{0.5}%
\psfrag{x30}[t][t]{1}%
\psfrag{x31}[t][t]{0}%
\psfrag{x32}[t][t]{0.5}%
\psfrag{x33}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[l][l]{20}%
\psfrag{v02}[l][l]{22}%
\psfrag{v03}[l][l]{24}%
\psfrag{v04}[l][l]{26}%
\psfrag{v05}[l][l]{28}%
\psfrag{v06}[l][l]{30}%
\psfrag{v07}[r][r]{0}%
\psfrag{v08}[r][r]{1}%
\psfrag{v09}[r][r]{2}%
\psfrag{v10}[r][r]{3}%
\psfrag{v11}[l][l]{20}%
\psfrag{v12}[l][l]{22}%
\psfrag{v13}[l][l]{24}%
\psfrag{v14}[l][l]{26}%
\psfrag{v15}[l][l]{28}%
\psfrag{v16}[l][l]{30}%
\psfrag{v17}[r][r]{0}%
\psfrag{v18}[r][r]{1}%
\psfrag{v19}[r][r]{2}%
\psfrag{v20}[r][r]{3}%
\psfrag{v21}[r][r]{4}%
\psfrag{v22}[r][r]{5}%
\psfrag{v23}[l][l]{20}%
\psfrag{v24}[l][l]{21}%
\psfrag{v25}[l][l]{22}%
\psfrag{v26}[l][l]{23}%
\psfrag{v27}[l][l]{24}%
\psfrag{v28}[r][r]{0}%
\psfrag{v29}[r][r]{0.2}%
\psfrag{v30}[r][r]{0.4}%
\psfrag{v31}[r][r]{0.6}%
\psfrag{v32}[r][r]{0.8}%
\psfrag{v33}[r][r]{1}%
\psfrag{v34}[l][l]{20}%
\psfrag{v35}[l][l]{21}%
\psfrag{v36}[l][l]{22}%
\psfrag{v37}[l][l]{23}%
\psfrag{v38}[l][l]{24}%
\psfrag{v39}[r][r]{0.2}%
\psfrag{v40}[r][r]{0.4}%
\psfrag{v41}[r][r]{0.6}%
\psfrag{v42}[r][r]{0.8}%
\psfrag{v43}[r][r]{1}%
\psfrag{v44}[r][r]{1.2}%
\psfrag{v45}[l][l]{20}%
\psfrag{v46}[l][l]{21}%
\psfrag{v47}[l][l]{22}%
\psfrag{v48}[l][l]{23}%
\psfrag{v49}[r][r]{1}%
\psfrag{v50}[r][r]{2}%
\psfrag{v51}[r][r]{3}%
\psfrag{v52}[r][r]{4}%
\psfrag{v53}[r][r]{5}%
\psfrag{v54}[r][r]{6}%
\psfrag{v55}[l][l]{10}%
\psfrag{v56}[l][l]{20}%
\psfrag{v57}[l][l]{30}%
\psfrag{v58}[l][l]{40}%
\psfrag{v59}[l][l]{50}%
\psfrag{v60}[l][l]{60}%
\psfrag{v61}[r][r]{0}%
\psfrag{v62}[r][r]{0.2}%
\psfrag{v63}[r][r]{0.4}%
\psfrag{v64}[r][r]{0.6}%
\psfrag{v65}[r][r]{0.8}%
\psfrag{v66}[r][r]{1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{flow_rule_h_1_2_3_4_5_6.matlab.eps}}%
\end{psfrags}%
%
% End flow_rule_h_1_2_3_4_5_6.matlab.tex


==> FiguresMatlab/flow_rule_hstop_fit_10_5_11_12.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\mu^b=0$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
\psfrag{s04}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\lambda=1$\end{tabular}}%
\psfrag{s05}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\mu^b=1$\end{tabular}}%
\psfrag{s08}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s09}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\mu^b=\infty$\end{tabular}}%
\psfrag{s11}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s12}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{5}%
\psfrag{x06}[t][t]{10}%
\psfrag{x07}[t][t]{15}%
\psfrag{x08}[t][t]{20}%
\psfrag{x09}[t][t]{0}%
\psfrag{x10}[t][t]{5}%
\psfrag{x11}[t][t]{10}%
\psfrag{x12}[t][t]{15}%
\psfrag{x13}[t][t]{20}%
\psfrag{x14}[t][t]{0}%
\psfrag{x15}[t][t]{2}%
\psfrag{x16}[t][t]{4}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{2}%
\psfrag{v03}[r][r]{4}%
\psfrag{v04}[r][r]{6}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{2}%
\psfrag{v07}[r][r]{4}%
\psfrag{v08}[r][r]{6}%
\psfrag{v09}[r][r]{0}%
\psfrag{v10}[r][r]{1}%
\psfrag{v11}[r][r]{2}%
\psfrag{v12}[r][r]{3}%
\psfrag{v13}[r][r]{4}%
\psfrag{v14}[r][r]{5}%
\psfrag{v15}[r][r]{0}%
\psfrag{v16}[r][r]{0.5}%
\psfrag{v17}[r][r]{1}%
\psfrag{v18}[r][r]{1.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{flow_rule_hstop_fit_10_5_11_12.matlab.eps}}%
\end{psfrags}%
%
% End flow_rule_hstop_fit_10_5_11_12.matlab.tex


==> FiguresMatlab/flow_rule_hstop_fit_1_2_3_4_5_6.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=0$\end{tabular}}%
\psfrag{s02}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\beta=3.302$\end{tabular}}%
\psfrag{s03}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1/2$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\beta=0.460$\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s07}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=2/3$\end{tabular}}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\beta=0.332$\end{tabular}}%
\psfrag{s09}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s10}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=5/6$\end{tabular}}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\beta=0.308$\end{tabular}}%
\psfrag{s12}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s13}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1$\end{tabular}}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\beta=0.288$\end{tabular}}%
\psfrag{s15}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s16}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=2$\end{tabular}}%
\psfrag{s17}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\beta=0.246$\end{tabular}}%
\psfrag{s18}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s19}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{10}%
\psfrag{x06}[t][t]{20}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{10}%
\psfrag{x09}[t][t]{20}%
\psfrag{x10}[t][t]{0}%
\psfrag{x11}[t][t]{10}%
\psfrag{x12}[t][t]{0}%
\psfrag{x13}[t][t]{10}%
\psfrag{x14}[t][t]{0}%
\psfrag{x15}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
\psfrag{v08}[r][r]{0}%
\psfrag{v09}[r][r]{1}%
\psfrag{v10}[r][r]{2}%
\psfrag{v11}[r][r]{3}%
\psfrag{v12}[r][r]{4}%
\psfrag{v13}[r][r]{5}%
\psfrag{v14}[r][r]{6}%
\psfrag{v15}[r][r]{7}%
\psfrag{v16}[r][r]{0}%
\psfrag{v17}[r][r]{1}%
\psfrag{v18}[r][r]{2}%
\psfrag{v19}[r][r]{3}%
\psfrag{v20}[r][r]{4}%
\psfrag{v21}[r][r]{5}%
\psfrag{v22}[r][r]{6}%
\psfrag{v23}[r][r]{7}%
\psfrag{v24}[r][r]{0}%
\psfrag{v25}[r][r]{1}%
\psfrag{v26}[r][r]{2}%
\psfrag{v27}[r][r]{3}%
\psfrag{v28}[r][r]{4}%
\psfrag{v29}[r][r]{0}%
\psfrag{v30}[r][r]{2}%
\psfrag{v31}[r][r]{4}%
\psfrag{v32}[r][r]{6}%
\psfrag{v33}[r][r]{8}%
\psfrag{v34}[r][r]{0}%
\psfrag{v35}[r][r]{2}%
\psfrag{v36}[r][r]{4}%
\psfrag{v37}[r][r]{6}%
\psfrag{v38}[r][r]{8}%
\psfrag{v39}[r][r]{10}%
\psfrag{v40}[r][r]{12}%
\psfrag{v41}[r][r]{14}%
%
% Figure:
\resizebox{16cm}{!}{\includegraphics{flow_rule_hstop_fit_1_2_3_4_5_6.matlab.eps}}%
\end{psfrags}%
%
% End flow_rule_hstop_fit_1_2_3_4_5_6.matlab.tex


==> FiguresMatlab/flow_rule_hstop_fit_compare_2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
\psfrag{s03}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{30}%
\psfrag{x05}[t][t]{40}%
\psfrag{x06}[t][t]{0}%
\psfrag{x07}[t][t]{5}%
\psfrag{x08}[t][t]{10}%
\psfrag{x09}[t][t]{15}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
\psfrag{v08}[r][r]{7}%
\psfrag{v09}[r][r]{8}%
\psfrag{v10}[r][r]{9}%
\psfrag{v11}[r][r]{0}%
\psfrag{v12}[r][r]{1}%
\psfrag{v13}[r][r]{2}%
\psfrag{v14}[r][r]{3}%
\psfrag{v15}[r][r]{4}%
\psfrag{v16}[r][r]{5}%
\psfrag{v17}[r][r]{6}%
\psfrag{v18}[r][r]{7}%
\psfrag{v19}[r][r]{8}%
\psfrag{v20}[r][r]{9}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{flow_rule_hstop_fit_compare_2.matlab.eps}}%
\end{psfrags}%
%
% End flow_rule_hstop_fit_compare_2.matlab.tex


==> FiguresMatlab/flow_rule_hstop_fit_compare_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
\psfrag{s03}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{40}%
\psfrag{x04}[t][t]{60}%
\psfrag{x05}[t][t]{80}%
\psfrag{x06}[t][t]{0}%
\psfrag{x07}[t][t]{10}%
\psfrag{x08}[t][t]{20}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
\psfrag{v08}[r][r]{7}%
\psfrag{v09}[r][r]{0}%
\psfrag{v10}[r][r]{1}%
\psfrag{v11}[r][r]{2}%
\psfrag{v12}[r][r]{3}%
\psfrag{v13}[r][r]{4}%
\psfrag{v14}[r][r]{5}%
\psfrag{v15}[r][r]{6}%
\psfrag{v16}[r][r]{7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{flow_rule_hstop_fit_compare_5.matlab.eps}}%
\end{psfrags}%
%
% End flow_rule_hstop_fit_compare_5.matlab.tex


==> FiguresMatlab/flow_rule_hstop_fit_jenkins_1_2_3_4_5_6.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\lambda=0$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
\psfrag{s04}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\lambda=1/2$\end{tabular}}%
\psfrag{s05}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\lambda=2/3$\end{tabular}}%
\psfrag{s08}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s09}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\lambda=5/6$\end{tabular}}%
\psfrag{s11}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s12}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\lambda=1$\end{tabular}}%
\psfrag{s14}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s15}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
\psfrag{s16}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}$\lambda=2$\end{tabular}}%
\psfrag{s17}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s18}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{50}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{50}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{50}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{20}%
\psfrag{x09}[t][t]{40}%
\psfrag{x10}[t][t]{0}%
\psfrag{x11}[t][t]{20}%
\psfrag{x12}[t][t]{40}%
\psfrag{x13}[t][t]{0}%
\psfrag{x14}[t][t]{50}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{2}%
\psfrag{v03}[r][r]{4}%
\psfrag{v04}[r][r]{6}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{2}%
\psfrag{v07}[r][r]{4}%
\psfrag{v08}[r][r]{6}%
\psfrag{v09}[r][r]{0}%
\psfrag{v10}[r][r]{2}%
\psfrag{v11}[r][r]{4}%
\psfrag{v12}[r][r]{6}%
\psfrag{v13}[r][r]{8}%
\psfrag{v14}[r][r]{0}%
\psfrag{v15}[r][r]{1}%
\psfrag{v16}[r][r]{2}%
\psfrag{v17}[r][r]{3}%
\psfrag{v18}[r][r]{4}%
\psfrag{v19}[r][r]{0}%
\psfrag{v20}[r][r]{2}%
\psfrag{v21}[r][r]{4}%
\psfrag{v22}[r][r]{6}%
\psfrag{v23}[r][r]{8}%
\psfrag{v24}[r][r]{0}%
\psfrag{v25}[r][r]{10}%
\psfrag{v26}[r][r]{20}%
\psfrag{v27}[r][r]{30}%
\psfrag{v28}[r][r]{40}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{flow_rule_hstop_fit_jenkins_1_2_3_4_5_6.matlab.eps}}%
\end{psfrags}%
%
% End flow_rule_hstop_fit_jenkins_1_2_3_4_5_6.matlab.tex


==> FiguresMatlab/flow_rule_hstop_fit_jenkins_3.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}L.63 \beta=0.138\end{tabular}}%
\psfrag{s03}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}h/h_{stop}(\tan(\theta)/\tan(\theta_1))^2\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}F\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{30}%
\psfrag{x05}[t][t]{40}%
\psfrag{x06}[t][t]{50}%
\psfrag{x07}[t][t]{60}%
\psfrag{x08}[t][t]{70}%
\psfrag{x09}[t][t]{80}%
%
% yticklabels:
\psfrag{v01}[l][l]{19}%
\psfrag{v02}[l][l]{20}%
\psfrag{v03}[l][l]{21}%
\psfrag{v04}[l][l]{22}%
\psfrag{v05}[l][l]{23}%
\psfrag{v06}[l][l]{24}%
\psfrag{v07}[l][l]{25}%
\psfrag{v08}[l][l]{26}%
\psfrag{v09}[l][l]{27}%
\psfrag{v10}[l][l]{28}%
\psfrag{v11}[l][l]{29}%
\psfrag{v12}[l][l]{30}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{2}%
\psfrag{v15}[r][r]{4}%
\psfrag{v16}[r][r]{6}%
\psfrag{v17}[r][r]{8}%
\psfrag{v18}[r][r]{10}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{flow_rule_hstop_fit_jenkins_3.matlab.eps}}%
\end{psfrags}%
%
% End flow_rule_hstop_fit_jenkins_3.matlab.tex


==> FiguresMatlab/flow_rule_hstop_fit_jenkins_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/h_s(\tan(\theta)/\tan(\theta_1))^2$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$F$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{30}%
\psfrag{x05}[t][t]{40}%
\psfrag{x06}[t][t]{50}%
\psfrag{x07}[t][t]{60}%
\psfrag{x08}[t][t]{70}%
\psfrag{x09}[t][t]{80}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
\psfrag{v08}[r][r]{7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{flow_rule_hstop_fit_jenkins_5.matlab.eps}}%
\end{psfrags}%
%
% End flow_rule_hstop_fit_jenkins_5.matlab.tex


==> FiguresMatlab/friction_1_2_3_4_5_6.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\mu$\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$(F+\gamma)/h$\end{tabular}}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=0$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1/2$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2/3$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=5/6$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1$}%
\psfrag{s15}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2$}%
\psfrag{s17}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s18}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.05}%
\psfrag{x03}[t][t]{0.1}%
\psfrag{x04}[t][t]{0.15}%
\psfrag{x05}[t][t]{0.2}%
\psfrag{x06}[t][t]{0.25}%
\psfrag{x07}[t][t]{0.3}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.35}%
\psfrag{v02}[r][r]{0.4}%
\psfrag{v03}[r][r]{0.45}%
\psfrag{v04}[r][r]{0.5}%
\psfrag{v05}[r][r]{0.55}%
\psfrag{v06}[r][r]{0.6}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{friction_1_2_3_4_5_6.matlab.eps}}%
\end{psfrags}%
%
% End friction_1_2_3_4_5_6.matlab.tex


==> FiguresMatlab/friction_2_5_6.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\mu$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1/2$\end{tabular}}%
\psfrag{s03}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$(F-\beta)/h$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1$\end{tabular}}%
\psfrag{s05}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$(F-\beta)/h$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=2$\end{tabular}}%
\psfrag{s07}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$(F-\beta)/h$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.05}%
\psfrag{x03}[t][t]{0.1}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{0.05}%
\psfrag{x06}[t][t]{0.1}%
\psfrag{x07}[t][t]{0.15}%
\psfrag{x08}[t][t]{0.2}%
\psfrag{x09}[t][t]{0}%
\psfrag{x10}[t][t]{0.05}%
\psfrag{x11}[t][t]{0.1}%
\psfrag{x12}[t][t]{0.15}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.35}%
\psfrag{v02}[r][r]{0.4}%
\psfrag{v03}[r][r]{0.45}%
\psfrag{v04}[r][r]{0.5}%
\psfrag{v05}[r][r]{0.55}%
\psfrag{v06}[r][r]{0.35}%
\psfrag{v07}[r][r]{0.4}%
\psfrag{v08}[r][r]{0.45}%
\psfrag{v09}[r][r]{0.5}%
\psfrag{v10}[r][r]{0.55}%
\psfrag{v11}[r][r]{0.6}%
\psfrag{v12}[r][r]{0.34}%
\psfrag{v13}[r][r]{0.36}%
\psfrag{v14}[r][r]{0.38}%
\psfrag{v15}[r][r]{0.4}%
\psfrag{v16}[r][r]{0.42}%
\psfrag{v17}[r][r]{0.44}%
\psfrag{v18}[r][r]{0.46}%
\psfrag{v19}[r][r]{0.48}%
\psfrag{v20}[r][r]{0.5}%
\psfrag{v21}[r][r]{0.52}%
\psfrag{v22}[r][r]{0.54}%
%
% Figure:
\resizebox{16cm}{!}{\includegraphics{friction_2_5_6.matlab.eps}}%
\end{psfrags}%
%
% End friction_2_5_6.matlab.tex


==> FiguresMatlab/hOverH_2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$H$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/H$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=20^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=21^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s15}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s16}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s18}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s19}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{10}%
\psfrag{x02}[t][t]{15}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{25}%
\psfrag{x05}[t][t]{30}%
\psfrag{x06}[t][t]{35}%
\psfrag{x07}[t][t]{40}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.85}%
\psfrag{v02}[r][r]{0.9}%
\psfrag{v03}[r][r]{0.95}%
\psfrag{v04}[r][r]{1}%
\psfrag{v05}[r][r]{1.05}%
\psfrag{v06}[r][r]{1.1}%
\psfrag{v07}[r][r]{1.15}%
\psfrag{v08}[r][r]{1.2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{hOverH_2.matlab.eps}}%
\end{psfrags}%
%
% End hOverH_2.matlab.tex


==> FiguresMatlab/hOverH_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$H$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h/H$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=20^\circ$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=20^\circ$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=22^\circ$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=23^\circ$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=24^\circ$}%
\psfrag{s12}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=25^\circ$}%
\psfrag{s13}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=26^\circ$}%
\psfrag{s14}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=27^\circ$}%
\psfrag{s15}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\theta=28^\circ$}%
\psfrag{s17}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s18}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{10}%
\psfrag{x02}[t][t]{15}%
\psfrag{x03}[t][t]{20}%
\psfrag{x04}[t][t]{25}%
\psfrag{x05}[t][t]{30}%
\psfrag{x06}[t][t]{35}%
\psfrag{x07}[t][t]{40}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.9}%
\psfrag{v02}[r][r]{0.92}%
\psfrag{v03}[r][r]{0.94}%
\psfrag{v04}[r][r]{0.96}%
\psfrag{v05}[r][r]{0.98}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{1.02}%
\psfrag{v08}[r][r]{1.04}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{hOverH_5.matlab.eps}}%
\end{psfrags}%
%
% End hOverH_5.matlab.tex


==> FiguresMatlab/ha_Alpha_1_2_3_4_5_6.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\alpha$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=0$}%
\psfrag{s06}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2$}%
\psfrag{s07}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1$}%
\psfrag{s08}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=5/6$}%
\psfrag{s09}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2/3$}%
\psfrag{s10}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1/2$}%
\psfrag{s11}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=0$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{8}{12}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{21}%
\psfrag{x02}[t][t]{22}%
\psfrag{x03}[t][t]{23}%
\psfrag{x04}[t][t]{24}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{26}%
\psfrag{x07}[t][t]{27}%
\psfrag{x08}[t][t]{28}%
%
% yticklabels:
\psfrag{v01}[r][r]{1}%
\psfrag{v02}[r][r]{1.05}%
\psfrag{v03}[r][r]{1.1}%
\psfrag{v04}[r][r]{1.15}%
\psfrag{v05}[r][r]{1.2}%
\psfrag{v06}[r][r]{1.25}%
\psfrag{v07}[r][r]{1.3}%
\psfrag{v08}[r][r]{1.35}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_Alpha_1_2_3_4_5_6.matlab.eps}}%
\end{psfrags}%
%
% End ha_Alpha_1_2_3_4_5_6.matlab.tex


==> FiguresMatlab/ha_K_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$K$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=40}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=10}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=20}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=30}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=40}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{22}%
\psfrag{x02}[t][t]{23}%
\psfrag{x03}[t][t]{24}%
\psfrag{x04}[t][t]{25}%
\psfrag{x05}[t][t]{26}%
\psfrag{x06}[t][t]{27}%
\psfrag{x07}[t][t]{28}%
\psfrag{x08}[t][t]{29}%
\psfrag{x09}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{1}%
\psfrag{v02}[r][r]{1.01}%
\psfrag{v03}[r][r]{1.02}%
\psfrag{v04}[r][r]{1.03}%
\psfrag{v05}[r][r]{1.04}%
\psfrag{v06}[r][r]{1.05}%
\psfrag{v07}[r][r]{1.06}%
\psfrag{v08}[r][r]{1.07}%
\psfrag{v09}[r][r]{1.08}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_K_5.matlab.eps}}%
\end{psfrags}%
%
% End ha_K_5.matlab.tex


==> FiguresMatlab/ha_K_5_2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$K$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1$\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$K$\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\lambda=1/2$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{22}%
\psfrag{x03}[t][t]{24}%
\psfrag{x04}[t][t]{26}%
\psfrag{x05}[t][t]{28}%
\psfrag{x06}[t][t]{20}%
\psfrag{x07}[t][t]{22}%
\psfrag{x08}[t][t]{24}%
\psfrag{x09}[t][t]{26}%
\psfrag{x10}[t][t]{28}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.6}%
\psfrag{v02}[r][r]{0.7}%
\psfrag{v03}[r][r]{0.8}%
\psfrag{v04}[r][r]{0.9}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{1.1}%
\psfrag{v07}[r][r]{1.2}%
\psfrag{v08}[r][r]{1.3}%
\psfrag{v09}[r][r]{0.99}%
\psfrag{v10}[r][r]{1}%
\psfrag{v11}[r][r]{1.01}%
\psfrag{v12}[r][r]{1.02}%
\psfrag{v13}[r][r]{1.03}%
\psfrag{v14}[r][r]{1.04}%
\psfrag{v15}[r][r]{1.05}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_K_5_2.matlab.eps}}%
\end{psfrags}%
%
% End ha_K_5_2.matlab.tex


==> FiguresMatlab/ha_Nu_2_3_4_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\bar\rho/\rho_p$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=30$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{21}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{23}%
\psfrag{x05}[t][t]{24}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{27}%
\psfrag{x09}[t][t]{28}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.48}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{0.52}%
\psfrag{v04}[r][r]{0.54}%
\psfrag{v05}[r][r]{0.56}%
\psfrag{v06}[r][r]{0.58}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.62}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_Nu_2_3_4_5.matlab.eps}}%
\end{psfrags}%
%
% End ha_Nu_2_3_4_5.matlab.tex


==> FiguresMatlab/ha_Nu_2_3_4_5_6.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\bar\rho/\rho_p$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1/2$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=5/6$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2/3$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1/2$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{21}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{23}%
\psfrag{x05}[t][t]{24}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{27}%
\psfrag{x09}[t][t]{28}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.52}%
\psfrag{v02}[r][r]{0.53}%
\psfrag{v03}[r][r]{0.54}%
\psfrag{v04}[r][r]{0.55}%
\psfrag{v05}[r][r]{0.56}%
\psfrag{v06}[r][r]{0.57}%
\psfrag{v07}[r][r]{0.58}%
\psfrag{v08}[r][r]{0.59}%
\psfrag{v09}[r][r]{0.6}%
\psfrag{v10}[r][r]{0.61}%
\psfrag{v11}[r][r]{0.62}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_Nu_2_3_4_5_6.matlab.eps}}%
\end{psfrags}%
%
% End ha_Nu_2_3_4_5_6.matlab.tex


==> FiguresMatlab/ha_Nu_3.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\bar\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=40}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=10}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=20}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=30}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=40}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{21}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{23}%
\psfrag{x05}[t][t]{24}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{27}%
\psfrag{x09}[t][t]{28}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.48}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{0.52}%
\psfrag{v04}[r][r]{0.54}%
\psfrag{v05}[r][r]{0.56}%
\psfrag{v06}[r][r]{0.58}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_Nu_3.matlab.eps}}%
\end{psfrags}%
%
% End ha_Nu_3.matlab.tex


==> FiguresMatlab/ha_Nu_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\bar\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=40}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=10}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=20}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=30}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=40}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{21}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{23}%
\psfrag{x05}[t][t]{24}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{27}%
\psfrag{x09}[t][t]{28}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.5}%
\psfrag{v02}[r][r]{0.51}%
\psfrag{v03}[r][r]{0.52}%
\psfrag{v04}[r][r]{0.53}%
\psfrag{v05}[r][r]{0.54}%
\psfrag{v06}[r][r]{0.55}%
\psfrag{v07}[r][r]{0.56}%
\psfrag{v08}[r][r]{0.57}%
\psfrag{v09}[r][r]{0.58}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_Nu_5.matlab.eps}}%
\end{psfrags}%
%
% End ha_Nu_5.matlab.tex


==> FiguresMatlab/ha_Nu_centre_2_3_4_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu_c$\end{tabular}}%
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s03}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\bar\nu$\end{tabular}}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=5/6$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=0$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1/2$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2/3$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=5/6$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{22}%
\psfrag{x03}[t][t]{24}%
\psfrag{x04}[t][t]{26}%
\psfrag{x05}[t][t]{28}%
\psfrag{x06}[t][t]{20}%
\psfrag{x07}[t][t]{22}%
\psfrag{x08}[t][t]{24}%
\psfrag{x09}[t][t]{26}%
\psfrag{x10}[t][t]{28}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.44}%
\psfrag{v02}[r][r]{0.46}%
\psfrag{v03}[r][r]{0.48}%
\psfrag{v04}[r][r]{0.5}%
\psfrag{v05}[r][r]{0.52}%
\psfrag{v06}[r][r]{0.54}%
\psfrag{v07}[r][r]{0.56}%
\psfrag{v08}[r][r]{0.58}%
\psfrag{v09}[r][r]{0.44}%
\psfrag{v10}[r][r]{0.46}%
\psfrag{v11}[r][r]{0.48}%
\psfrag{v12}[r][r]{0.5}%
\psfrag{v13}[r][r]{0.52}%
\psfrag{v14}[r][r]{0.54}%
\psfrag{v15}[r][r]{0.56}%
\psfrag{v16}[r][r]{0.58}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_Nu_centre_2_3_4_5.matlab.eps}}%
\end{psfrags}%
%
% End ha_Nu_centre_2_3_4_5.matlab.tex


==> FiguresMatlab/ha_alpha_3.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\alpha$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold profile}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=10}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=20}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=30}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=40}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Linear profile}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold profile}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{21}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{23}%
\psfrag{x05}[t][t]{24}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{27}%
\psfrag{x09}[t][t]{28}%
%
% yticklabels:
\psfrag{v01}[r][r]{1.16}%
\psfrag{v02}[r][r]{1.18}%
\psfrag{v03}[r][r]{1.2}%
\psfrag{v04}[r][r]{1.22}%
\psfrag{v05}[r][r]{1.24}%
\psfrag{v06}[r][r]{1.26}%
\psfrag{v07}[r][r]{1.28}%
\psfrag{v08}[r][r]{1.3}%
\psfrag{v09}[r][r]{1.32}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_alpha_3.matlab.eps}}%
\end{psfrags}%
%
% End ha_alpha_3.matlab.tex


==> FiguresMatlab/ha_alpha_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\alpha$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold profile}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=10}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=20}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=30}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=40}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Linear profile}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Bagnold profile}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{21}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{23}%
\psfrag{x05}[t][t]{24}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{27}%
\psfrag{x09}[t][t]{28}%
%
% yticklabels:
\psfrag{v01}[r][r]{1.25}%
\psfrag{v02}[r][r]{1.3}%
\psfrag{v03}[r][r]{1.35}%
\psfrag{v04}[r][r]{1.4}%
\psfrag{v05}[r][r]{1.45}%
\psfrag{v06}[r][r]{1.5}%
\psfrag{v07}[r][r]{1.55}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_alpha_5.matlab.eps}}%
\end{psfrags}%
%
% End ha_alpha_5.matlab.tex


==> FiguresMatlab/ha_bottom_friction_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta-\tan^{-1}(\mu)$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=40}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=10}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=20}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=30}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}H=40}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{21}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{23}%
\psfrag{x05}[t][t]{24}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{27}%
\psfrag{x09}[t][t]{28}%
\psfrag{x10}[t][t]{29}%
\psfrag{x11}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{ha_bottom_friction_5.matlab.eps}}%
\end{psfrags}%
%
% End ha_bottom_friction_5.matlab.tex


==> FiguresMatlab/hstop_diagram_10.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h_s(\theta)$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}arrested}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}flowing}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h_s(\theta)$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{18.5}%
\psfrag{x02}[t][t]{19}%
\psfrag{x03}[t][t]{19.5}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{20.5}%
\psfrag{x06}[t][t]{21}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
\psfrag{v09}[r][r]{40}%
\psfrag{v10}[r][r]{45}%
\psfrag{v11}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{hstop_diagram_10.matlab.eps}}%
\end{psfrags}%
%
% End hstop_diagram_10.matlab.tex


==> FiguresMatlab/hstop_diagram_10_5_11_12.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu^b=\infty$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu^b=0$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu^b=1$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu^b=\infty$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{22}%
\psfrag{x03}[t][t]{24}%
\psfrag{x04}[t][t]{26}%
\psfrag{x05}[t][t]{28}%
\psfrag{x06}[t][t]{30}%
\psfrag{x07}[t][t]{32}%
\psfrag{x08}[t][t]{34}%
\psfrag{x09}[t][t]{36}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
\psfrag{v09}[r][r]{40}%
\psfrag{v10}[r][r]{45}%
\psfrag{v11}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{hstop_diagram_10_5_11_12.matlab.eps}}%
\end{psfrags}%
%
% End hstop_diagram_10_5_11_12.matlab.tex


==> FiguresMatlab/hstop_diagram_1_2_3_4_5_6.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=0$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1/2$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2/3$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=5/6$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=2$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{15}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{25}%
\psfrag{x04}[t][t]{30}%
\psfrag{x05}[t][t]{35}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
\psfrag{v09}[r][r]{40}%
\psfrag{v10}[r][r]{45}%
\psfrag{v11}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{hstop_diagram_1_2_3_4_5_6.matlab.eps}}%
\end{psfrags}%
%
% End hstop_diagram_1_2_3_4_5_6.matlab.tex


==> FiguresMatlab/hstop_diagram_2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s03}[r][r]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{r}$\delta_3^{1/2}\rightarrow$\end{tabular}}%
\psfrag{s04}[r][r]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{r}$\delta_{acc}^{1/2}\rightarrow$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{19}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{21}%
\psfrag{x04}[t][t]{22}%
\psfrag{x05}[t][t]{23}%
\psfrag{x06}[t][t]{24}%
\psfrag{x07}[t][t]{25}%
\psfrag{x08}[t][t]{26}%
\psfrag{x09}[t][t]{27}%
\psfrag{x10}[t][t]{28}%
\psfrag{x11}[t][t]{29}%
\psfrag{x12}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{5}%
\psfrag{v02}[r][r]{10}%
\psfrag{v03}[r][r]{15}%
\psfrag{v04}[r][r]{20}%
\psfrag{v05}[r][r]{25}%
\psfrag{v06}[r][r]{30}%
\psfrag{v07}[r][r]{35}%
\psfrag{v08}[r][r]{40}%
\psfrag{v09}[r][r]{45}%
\psfrag{v10}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{hstop_diagram_2.matlab.eps}}%
\end{psfrags}%
%
% End hstop_diagram_2.matlab.tex


==> FiguresMatlab/hstop_diagram_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h_s(\theta)$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}arrested}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}flowing}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$h_s(\theta)$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{19}%
\psfrag{x02}[t][t]{20}%
\psfrag{x03}[t][t]{21}%
\psfrag{x04}[t][t]{22}%
\psfrag{x05}[t][t]{23}%
\psfrag{x06}[t][t]{24}%
\psfrag{x07}[t][t]{25}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
\psfrag{v09}[r][r]{40}%
\psfrag{v10}[r][r]{45}%
\psfrag{v11}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{hstop_diagram_5.matlab.eps}}%
\end{psfrags}%
%
% End hstop_diagram_5.matlab.tex


==> FiguresMatlab/hstop_diagram_7_5_8_9.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$h$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu=\infty$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu=0$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\lambda=1$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu=1$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\mu=\infty$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{5}%
\psfrag{x02}[t][t]{10}%
\psfrag{x03}[t][t]{15}%
\psfrag{x04}[t][t]{20}%
\psfrag{x05}[t][t]{25}%
\psfrag{x06}[t][t]{30}%
\psfrag{x07}[t][t]{35}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{15}%
\psfrag{v05}[r][r]{20}%
\psfrag{v06}[r][r]{25}%
\psfrag{v07}[r][r]{30}%
\psfrag{v08}[r][r]{35}%
\psfrag{v09}[r][r]{40}%
\psfrag{v10}[r][r]{45}%
\psfrag{v11}[r][r]{50}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{hstop_diagram_7_5_8_9.matlab.eps}}%
\end{psfrags}%
%
% End hstop_diagram_7_5_8_9.matlab.tex


==> FiguresMatlab/oscillating.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z/h$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}t=2000}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}t=600}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}t=2000}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{oscillating.matlab.eps}}%
\end{psfrags}%
%
% End oscillating.matlab.tex


==> FiguresMatlab/rho_fit_full_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\bar\rho/\rho_p$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\bar\rho_c/\rho_p$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\rho_c^{fit}/\rho_p$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=30$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{21}%
\psfrag{x03}[t][t]{22}%
\psfrag{x04}[t][t]{23}%
\psfrag{x05}[t][t]{24}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{26}%
\psfrag{x08}[t][t]{27}%
\psfrag{x09}[t][t]{28}%
\psfrag{x10}[t][t]{29}%
\psfrag{x11}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.35}%
\psfrag{v02}[r][r]{0.4}%
\psfrag{v03}[r][r]{0.45}%
\psfrag{v04}[r][r]{0.5}%
\psfrag{v05}[r][r]{0.55}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{rho_fit_full_5.matlab.eps}}%
\end{psfrags}%
%
% End rho_fit_full_5.matlab.tex


==> FiguresMatlab/t_dependence_momeq.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=200$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=1$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=5$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=10$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=50$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=100$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=200$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.2}%
\psfrag{v02}[r][r]{-0.1}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{0.1}%
\psfrag{v05}[r][r]{0.2}%
\psfrag{v06}[r][r]{0.3}%
\psfrag{v07}[r][r]{0.4}%
\psfrag{v08}[r][r]{0.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{t_dependence_momeq.matlab.eps}}%
\end{psfrags}%
%
% End t_dependence_momeq.matlab.tex


==> FiguresMatlab/t_dependence_momeq_direct.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=10$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=10$}%
\psfrag{s08}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
\psfrag{x08}[t][t]{-5}%
\psfrag{x09}[t][t]{0}%
\psfrag{x10}[t][t]{5}%
\psfrag{x11}[t][t]{10}%
\psfrag{x12}[t][t]{15}%
\psfrag{x13}[t][t]{20}%
\psfrag{x14}[t][t]{25}%
\psfrag{x15}[t][t]{30}%
\psfrag{x16}[t][t]{35}%
\psfrag{x17}[t][t]{-5}%
\psfrag{x18}[t][t]{0}%
\psfrag{x19}[t][t]{5}%
\psfrag{x20}[t][t]{10}%
\psfrag{x21}[t][t]{15}%
\psfrag{x22}[t][t]{20}%
\psfrag{x23}[t][t]{25}%
\psfrag{x24}[t][t]{30}%
\psfrag{x25}[t][t]{35}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.01}%
\psfrag{v02}[r][r]{0}%
\psfrag{v03}[r][r]{0.01}%
\psfrag{v04}[r][r]{-0.02}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{0.02}%
\psfrag{v07}[r][r]{-0.2}%
\psfrag{v08}[r][r]{0}%
\psfrag{v09}[r][r]{0.2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{t_dependence_momeq_direct.matlab.eps}}%
\end{psfrags}%
%
% End t_dependence_momeq_direct.matlab.tex


==> FiguresMatlab/t_dependence_nu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=200$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=10$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=50$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=100$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=200$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.4}%
\psfrag{v02}[r][r]{0.45}%
\psfrag{v03}[r][r]{0.5}%
\psfrag{v04}[r][r]{0.55}%
\psfrag{v05}[r][r]{0.6}%
\psfrag{v06}[r][r]{0.65}%
\psfrag{v07}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{t_dependence_nu.matlab.eps}}%
\end{psfrags}%
%
% End t_dependence_nu.matlab.tex


==> FiguresMatlab/table_fittingfull5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\bar\rho$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=40$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=30$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=20$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$H=10$}%
\psfrag{s11}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s12}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\alpha$\end{tabular}}%
\psfrag{s15}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s16}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s17}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\theta$\end{tabular}}%
\psfrag{s18}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$K$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{20}%
\psfrag{x02}[t][t]{22}%
\psfrag{x03}[t][t]{24}%
\psfrag{x04}[t][t]{26}%
\psfrag{x05}[t][t]{28}%
\psfrag{x06}[t][t]{22}%
\psfrag{x07}[t][t]{24}%
\psfrag{x08}[t][t]{26}%
\psfrag{x09}[t][t]{28}%
\psfrag{x10}[t][t]{22}%
\psfrag{x11}[t][t]{24}%
\psfrag{x12}[t][t]{26}%
\psfrag{x13}[t][t]{28}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.99}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{1.01}%
\psfrag{v04}[r][r]{1.02}%
\psfrag{v05}[r][r]{1.03}%
\psfrag{v06}[r][r]{1.04}%
\psfrag{v07}[r][r]{1.05}%
\psfrag{v08}[r][r]{1.25}%
\psfrag{v09}[r][r]{1.3}%
\psfrag{v10}[r][r]{1.35}%
\psfrag{v11}[r][r]{1.4}%
\psfrag{v12}[r][r]{1.45}%
\psfrag{v13}[r][r]{0.51}%
\psfrag{v14}[r][r]{0.52}%
\psfrag{v15}[r][r]{0.53}%
\psfrag{v16}[r][r]{0.54}%
\psfrag{v17}[r][r]{0.55}%
\psfrag{v18}[r][r]{0.56}%
\psfrag{v19}[r][r]{0.57}%
\psfrag{v20}[r][r]{0.58}%
%
% Figure:
\resizebox{16cm}{!}{\includegraphics{table_fittingfull5.matlab.eps}}%
\end{psfrags}%
%
% End table_fittingfull5.matlab.tex


==> FiguresMatlab/u_fit_5.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=10,A=23,bfit=5.0566\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=10,A=24,bfit=3.7648\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=10,A=25,bfit=2.8279\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=10,A=26,bfit=2.1313\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=10,A=27,bfit=1.5813\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=10,A=28,bfit=1.1317\end{tabular}}%
\psfrag{s07}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=20,A=22,bfit=3.5014\end{tabular}}%
\psfrag{s08}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=20,A=23,bfit=2.5504\end{tabular}}%
\psfrag{s09}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=20,A=24,bfit=1.9085\end{tabular}}%
\psfrag{s10}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=20,A=25,bfit=1.4422\end{tabular}}%
\psfrag{s11}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=20,A=26,bfit=1.0893\end{tabular}}%
\psfrag{s12}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=20,A=27,bfit=0.81074\end{tabular}}%
\psfrag{s13}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=20,A=28,bfit=0.58507\end{tabular}}%
\psfrag{s14}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=30,A=20,bfit=5.2687\end{tabular}}%
\psfrag{s15}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=30,A=22,bfit=2.3376\end{tabular}}%
\psfrag{s16}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=30,A=23,bfit=1.7078\end{tabular}}%
\psfrag{s17}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=30,A=24,bfit=1.2769\end{tabular}}%
\psfrag{s18}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=30,A=25,bfit=0.96562\end{tabular}}%
\psfrag{s19}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=30,A=26,bfit=0.72916\end{tabular}}%
\psfrag{s20}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=30,A=27,bfit=0.54408\end{tabular}}%
\psfrag{s21}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=30,A=28,bfit=0.39405\end{tabular}}%
\psfrag{s22}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=40,A=20,bfit=3.9669\end{tabular}}%
\psfrag{s23}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=40,A=22,bfit=1.7534\end{tabular}}%
\psfrag{s24}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=40,A=24,bfit=0.95861\end{tabular}}%
\psfrag{s25}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=40,A=26,bfit=0.54727\end{tabular}}%
\psfrag{s26}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}H=40,A=28,bfit=0.29779\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{0.5}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{0}%
\psfrag{x08}[t][t]{0.5}%
\psfrag{x09}[t][t]{1}%
\psfrag{x10}[t][t]{0}%
\psfrag{x11}[t][t]{0.5}%
\psfrag{x12}[t][t]{1}%
\psfrag{x13}[t][t]{0}%
\psfrag{x14}[t][t]{0.5}%
\psfrag{x15}[t][t]{1}%
\psfrag{x16}[t][t]{0}%
\psfrag{x17}[t][t]{0.5}%
\psfrag{x18}[t][t]{1}%
\psfrag{x19}[t][t]{0}%
\psfrag{x20}[t][t]{0.5}%
\psfrag{x21}[t][t]{1}%
\psfrag{x22}[t][t]{0}%
\psfrag{x23}[t][t]{0.5}%
\psfrag{x24}[t][t]{1}%
\psfrag{x25}[t][t]{0}%
\psfrag{x26}[t][t]{0.5}%
\psfrag{x27}[t][t]{1}%
\psfrag{x28}[t][t]{0}%
\psfrag{x29}[t][t]{0.5}%
\psfrag{x30}[t][t]{1}%
\psfrag{x31}[t][t]{0}%
\psfrag{x32}[t][t]{0.5}%
\psfrag{x33}[t][t]{1}%
\psfrag{x34}[t][t]{0}%
\psfrag{x35}[t][t]{0.5}%
\psfrag{x36}[t][t]{1}%
\psfrag{x37}[t][t]{0}%
\psfrag{x38}[t][t]{0.5}%
\psfrag{x39}[t][t]{1}%
\psfrag{x40}[t][t]{0}%
\psfrag{x41}[t][t]{0.5}%
\psfrag{x42}[t][t]{1}%
\psfrag{x43}[t][t]{0}%
\psfrag{x44}[t][t]{0.5}%
\psfrag{x45}[t][t]{1}%
\psfrag{x46}[t][t]{0}%
\psfrag{x47}[t][t]{0.5}%
\psfrag{x48}[t][t]{1}%
\psfrag{x49}[t][t]{0}%
\psfrag{x50}[t][t]{0.5}%
\psfrag{x51}[t][t]{1}%
\psfrag{x52}[t][t]{0}%
\psfrag{x53}[t][t]{0.5}%
\psfrag{x54}[t][t]{1}%
\psfrag{x55}[t][t]{0}%
\psfrag{x56}[t][t]{0.5}%
\psfrag{x57}[t][t]{1}%
\psfrag{x58}[t][t]{0}%
\psfrag{x59}[t][t]{0.5}%
\psfrag{x60}[t][t]{1}%
\psfrag{x61}[t][t]{0}%
\psfrag{x62}[t][t]{0.5}%
\psfrag{x63}[t][t]{1}%
\psfrag{x64}[t][t]{0}%
\psfrag{x65}[t][t]{0.5}%
\psfrag{x66}[t][t]{1}%
\psfrag{x67}[t][t]{0}%
\psfrag{x68}[t][t]{0.5}%
\psfrag{x69}[t][t]{1}%
\psfrag{x70}[t][t]{0}%
\psfrag{x71}[t][t]{0.5}%
\psfrag{x72}[t][t]{1}%
\psfrag{x73}[t][t]{0}%
\psfrag{x74}[t][t]{0.5}%
\psfrag{x75}[t][t]{1}%
\psfrag{x76}[t][t]{0}%
\psfrag{x77}[t][t]{0.5}%
\psfrag{x78}[t][t]{1}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{0}%
\psfrag{v05}[r][r]{1}%
\psfrag{v06}[r][r]{2}%
\psfrag{v07}[r][r]{0}%
\psfrag{v08}[r][r]{1}%
\psfrag{v09}[r][r]{2}%
\psfrag{v10}[r][r]{0}%
\psfrag{v11}[r][r]{1}%
\psfrag{v12}[r][r]{2}%
\psfrag{v13}[r][r]{0}%
\psfrag{v14}[r][r]{1}%
\psfrag{v15}[r][r]{2}%
\psfrag{v16}[r][r]{0}%
\psfrag{v17}[r][r]{1}%
\psfrag{v18}[r][r]{2}%
\psfrag{v19}[r][r]{0}%
\psfrag{v20}[r][r]{1}%
\psfrag{v21}[r][r]{2}%
\psfrag{v22}[r][r]{0}%
\psfrag{v23}[r][r]{1}%
\psfrag{v24}[r][r]{2}%
\psfrag{v25}[r][r]{0}%
\psfrag{v26}[r][r]{1}%
\psfrag{v27}[r][r]{2}%
\psfrag{v28}[r][r]{0}%
\psfrag{v29}[r][r]{1}%
\psfrag{v30}[r][r]{2}%
\psfrag{v31}[r][r]{0}%
\psfrag{v32}[r][r]{1}%
\psfrag{v33}[r][r]{2}%
\psfrag{v34}[r][r]{0}%
\psfrag{v35}[r][r]{1}%
\psfrag{v36}[r][r]{2}%
\psfrag{v37}[r][r]{0}%
\psfrag{v38}[r][r]{1}%
\psfrag{v39}[r][r]{2}%
\psfrag{v40}[r][r]{0}%
\psfrag{v41}[r][r]{1}%
\psfrag{v42}[r][r]{2}%
\psfrag{v43}[r][r]{0}%
\psfrag{v44}[r][r]{1}%
\psfrag{v45}[r][r]{2}%
\psfrag{v46}[r][r]{0}%
\psfrag{v47}[r][r]{1}%
\psfrag{v48}[r][r]{2}%
\psfrag{v49}[r][r]{0}%
\psfrag{v50}[r][r]{1}%
\psfrag{v51}[r][r]{2}%
\psfrag{v52}[r][r]{0}%
\psfrag{v53}[r][r]{1}%
\psfrag{v54}[r][r]{2}%
\psfrag{v55}[r][r]{0}%
\psfrag{v56}[r][r]{1}%
\psfrag{v57}[r][r]{2}%
\psfrag{v58}[r][r]{0}%
\psfrag{v59}[r][r]{1}%
\psfrag{v60}[r][r]{2}%
\psfrag{v61}[r][r]{0}%
\psfrag{v62}[r][r]{1}%
\psfrag{v63}[r][r]{2}%
\psfrag{v64}[r][r]{0}%
\psfrag{v65}[r][r]{1}%
\psfrag{v66}[r][r]{2}%
\psfrag{v67}[r][r]{0}%
\psfrag{v68}[r][r]{1}%
\psfrag{v69}[r][r]{2}%
\psfrag{v70}[r][r]{0}%
\psfrag{v71}[r][r]{1}%
\psfrag{v72}[r][r]{2}%
\psfrag{v73}[r][r]{0}%
\psfrag{v74}[r][r]{1}%
\psfrag{v75}[r][r]{2}%
\psfrag{v76}[r][r]{0}%
\psfrag{v77}[r][r]{1}%
\psfrag{v78}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{u_fit_5.matlab.eps}}%
\end{psfrags}%
%
% End u_fit_5.matlab.tex


==> Images/HamiltonianSystem.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5102.00,4534.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(990,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(990,1298){\makebox(0,0)[r]{\strut{} 1e-09}}%
      \put(990,1892){\makebox(0,0)[r]{\strut{} 2e-09}}%
      \put(990,2487){\makebox(0,0)[r]{\strut{} 3e-09}}%
      \put(990,3081){\makebox(0,0)[r]{\strut{} 4e-09}}%
      \put(990,3675){\makebox(0,0)[r]{\strut{} 5e-09}}%
      \put(990,4269){\makebox(0,0)[r]{\strut{} 6e-09}}%
      \put(1122,484){\makebox(0,0){\strut{} 0}}%
      \put(1570,484){\makebox(0,0){\strut{} 2e-07}}%
      \put(2018,484){\makebox(0,0){\strut{} 4e-07}}%
      \put(2466,484){\makebox(0,0){\strut{} 6e-07}}%
      \put(2914,484){\makebox(0,0){\strut{} 8e-07}}%
      \put(3361,484){\makebox(0,0){\strut{} 1e-06}}%
      \put(3809,484){\makebox(0,0){\strut{} 1.2e-06}}%
      \put(4257,484){\makebox(0,0){\strut{} 1.4e-06}}%
      \put(4705,484){\makebox(0,0){\strut{} 1.6e-06}}%
      \put(2913,154){\makebox(0,0){\strut{}t}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3718,4096){\makebox(0,0)[r]{\strut{}$E_{kin}+E_{spring}$}}%
      \csname LTb\endcsname%
      \put(3718,3876){\makebox(0,0)[r]{\strut{}$E_{kin}$}}%
      \csname LTb\endcsname%
      \put(3718,3656){\makebox(0,0)[r]{\strut{}$E_{spring}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{HamiltonianSystem}}%
    \gplfronttext
  \end{picture}%
\endgroup

